Combining Shrinkage and Sparsity in Conjugate Vector Autoregressive Models

Conjugate priors allow for fast inference in large dimensional vector autoregressive (VAR) models but, at the same time, introduce the restriction that each equation features the same set of explanatory variables. This paper proposes a straightforward means of post-processing posterior estimates of a conjugate Bayesian VAR to effectively perform equation-specific covariate selection. Compared to existing techniques using shrinkage alone, our approach combines shrinkage and sparsity in both the VAR coefficients and the error variance-covariance matrices, greatly reducing estimation uncertainty in large dimensions while maintaining computational tractability. We illustrate our approach by means of two applications. The first application uses synthetic data to investigate the properties of the model across different data-generating processes, the second application analyzes the predictive gains from sparsification in a forecasting exercise for US data.

==> CRPS_final.tex <==
%latex.default(lps.all, file = paste0(score.type, "_", eval.type,     ".tex"), title = "", ctable = FALSE, rgroupTexCmd = "scshape",     n.cgroup = n.cgroup, cgroup = cgroup, colheads = colheads,     rgroup = rgroup, n.rgroup = n.rgroup, caption = "", label = "tab:dens",     size = "tiny", rownamesTexCmd = my.rownamesTexCmd, booktabs = TRUE,     rowname = "", numeric.dollar = FALSE, caption.loc = "bottom",     landscape = TRUE)%
\begin{landscape}\begin{table}[!tbp]
{\tiny
\begin{center}
\scalebox{0.95}{
\begin{tabular}{llclllclllclllclll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{1}{c}{\bfseries Spec.}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Avg.}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal 1-step-ahead}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal 4-step-ahead}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal 8-step-ahead}\tabularnewline
\cline{2-2} \cline{4-6} \cline{8-10} \cline{12-14} \cline{16-18}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{1-step ahead}&\multicolumn{1}{c}{4-step ahead}&\multicolumn{1}{c}{8-step ahead}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{ CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{ CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}\tabularnewline
\midrule
{\scshape Small}&&&&&&&&&&&&&&&&&\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   0.984&   1.002&   0.989&   &   0.997&   \textbf{0.980}&   0.975&   &   1.011&   0.986&   1.023&   &   0.979&   0.989&   1.002\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   0.971&   0.996&   0.981***&   &   0.986&   0.990&   0.917*&   &   1.008&   0.999&   0.971&   &   0.959**&   0.993&   0.984\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   \textbf{0.967}&   0.982&   0.986&   &   0.992&   1.000&   0.876**&   &   0.979&   0.987&   0.973&   &   0.982&   0.983&   1.000\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   0.976&   0.976&   0.971***&   &   0.997&   1.021&   0.867**&   &   0.976&   0.994&   0.940&   &   0.963*&   0.975*&   0.974\tabularnewline
\shadeRow   ~~&   SSVS&   &   1.003&   1.025*&   1.016**&   &   1.018&   0.984&   1.017&   &   1.044&   1.013&   1.026&   &   1.034**&   0.984&   1.061***\tabularnewline
\midrule
{\scshape FAVAR}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.013&   1.031**&   1.008&   &   0.956&   1.052*&   1.018&   &   1.069**&   1.025&   0.994&   &   1.070*&   0.980&   0.983\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   0.997&   1.015&   0.999&   &   0.939&   1.038&   0.998&   &   1.036&   1.018&   0.982&   &   0.990&   0.996&   1.016\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   0.996&   1.012&   0.978**&   &   0.939&   1.062&   0.951&   &   1.068*&   0.990&   0.985&   &   0.973&   0.972*&   0.997\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.010&   1.010&   0.982**&   &   0.943&   1.095&   0.946&   &   1.076&   \textbf{0.971}&   1.002&   &   0.964*&   0.992&   0.987\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   1.022&   0.997&   0.983&   &   0.937&   1.118&   0.959&   &   1.009&   0.992&   0.993&   &   0.952**&   0.994&   1.001\tabularnewline
\shadeRow   ~~&   SSVS&   &   1.284***&   1.275***&   1.263***&   &   0.922&   1.583***&   1.214**&   &   1.112***&   1.454***&   1.124*&   &   1.072**&   1.424***&   1.184***\tabularnewline
\midrule
{\scshape Medium}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.020&   0.998&   1.011&   &   0.881**&   1.136*&   0.992&   &   1.020&   0.982&   1.003&   &   1.027&   0.993&   1.027\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   1.001&   0.968&   0.981&   &   0.868***&   1.145*&   0.911&   &   0.972&   0.977&   0.947&   &   0.976&   0.988&   0.972\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   0.974&   0.967&   0.958***&   &   \textbf{0.859***}&   1.138*&   0.830***&   &   0.965&   0.986&   0.934&   &   0.950&   0.979&   0.925***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   0.972&   0.954&   0.933***&   &   0.928**&   1.091&   0.814***&   &   0.958&   0.983&   0.889*&   &   0.931***&   \textbf{0.956***}&   0.887***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   0.988&   0.947*&   0.951***&   &   0.972&   1.091&   0.823***&   &   0.951&   0.984&   0.869**&   &   0.942**&   0.984&   0.893***\tabularnewline
\shadeRow   ~~&   SSVS&   &   1.339***&   1.315***&   1.356***&   &   0.980&   1.653***&   1.235***&   &   1.132***&   1.482***&   1.213**&   &   1.178*&   1.474***&   1.349**\tabularnewline
\midrule
{\scshape Large ($\theta_1 = 0.025$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.001&   0.986&   0.983&   &   0.895**&   1.105&   0.950&   &   1.004&   0.981&   0.972&   &   0.999&   0.974**&   0.980\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   1.020&   0.955&   0.955***&   &   0.969&   1.134*&   0.882**&   &   0.966&   0.974&   0.903*&   &   0.945**&   0.979*&   0.916***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   1.034&   0.958&   0.955***&   &   0.993&   1.125&   0.922&   &   0.973&   0.983&   0.886**&   &   0.945*&   0.979&   0.920**\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.025&   0.957&   0.955***&   &   1.005&   1.103&   0.910&   &   0.959&   0.988&   0.894*&   &   0.925***&   0.988&   0.924***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   1.034&   0.963&   0.950***&   &   1.006&   1.117&   0.921&   &   0.969&   0.994&   0.891**&   &   0.935***&   0.973*&   0.922**\tabularnewline
\midrule
{\scshape Large ($\theta_1 = 0.050$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.003&   0.994&   0.989&   &   0.922&   1.081&   0.966&   &   1.026&   0.980&   0.982&   &   1.009&   0.984&   0.972\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   0.985&   0.948*&   0.938***&   &   0.903***&   1.128&   0.834***&   &   0.955&   0.984&   0.865**&   &   0.936***&   0.969*&   0.874***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   1.015&   0.940**&   0.933***&   &   0.970&   1.140*&   0.849**&   &   0.949&   0.989&   0.828***&   &   0.926**&   0.985&   0.830***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.002&   0.940**&   0.932***&   &   0.980&   1.108&   0.840**&   &   0.947&   0.995&   0.820***&   &   0.924**&   0.980&   0.842***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   1.005&   0.939**&   0.932***&   &   0.980&   1.115&   0.840**&   &   0.944&   0.994&   0.821***&   &   0.925**&   0.978*&   0.844***\tabularnewline
\midrule
{\scshape Large ($\theta_1 = 0.075$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.017&   1.001&   1.024&   &   0.943&   1.085&   0.989&   &   1.020&   0.988&   1.000&   &   1.073*&   0.993&   1.022\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   0.995&   0.935***&   0.934***&   &   0.905**&   1.146*&   0.841***&   &   0.944**&   0.980&   0.833***&   &   0.923***&   0.980&   0.854***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   0.993&   0.930**&   0.928***&   &   0.965&   1.133*&   0.780***&   &   0.948&   0.992&   0.778***&   &   0.915**&   0.993&   0.809***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.003&   \textbf{0.920**}&   0.926***&   &   1.016&   1.114&   0.790***&   &   \textbf{0.930}&   0.991&   \textbf{0.762***}&   &   0.928*&   0.998&   \textbf{0.771***}\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   0.995&   0.930**&   \textbf{0.925***}&   &   0.987&   1.122&   \textbf{0.780***}&   &   0.956&   0.989&   0.778***&   &   \textbf{0.909***}&   1.000&   0.791***\tabularnewline
\bottomrule
\end{tabular}}
\caption{CRPS ratios relative to the \textit{small-scale} BVAR with a Minnesota prior. \label{tab:CRPS}}
\begin{minipage}{\linewidth}
\footnotesize \textbf{Notes}: Bold numbers indicate lowest CRPS ratios for each horizon and target variable (and therefore best performing models over the full hold-out sample in terms of density forecasts). Gray shaded rows denote non-sparsified models. Asterisks indicate statistical significance for each model relative to the benchmark at the $1$ ($^{***}$), $5$ ($^{**}$) and $10$ ($^{*}$) percent significance levels. 
\end{minipage}\end{center}}
\end{table}\end{landscape}


==> CRPS_final_rank.tex <==
%latex.default(crps.all, file = paste0("CRPS", "_", eval.type,     ".tex"), title = "", ctable = FALSE, rgroupTexCmd = "scshape",     n.cgroup = n.cgroup, cgroup = cgroup, colheads = colheads,     rgroup = rgroup, n.rgroup = n.rgroup, caption = "", label = "tab:point",     size = "tiny", rownamesTexCmd = my.rownamesTexCmd, rowname = "",     booktabs = TRUE, numeric.dollar = TRUE, caption.loc = "bottom",     landscape = TRUE)%
\begin{table}[!htp]
{\tiny
\begin{center}
\scalebox{0.9}{
\begin{tabular}{llclllclllclllclll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{1}{c}{\bfseries Spec.}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Avg.}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal One-quarter-ahead}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal One-year-ahead}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal Two-year-ahead}\tabularnewline
\cline{2-2} \cline{4-6} \cline{8-10} \cline{12-14} \cline{16-18}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{One-quarter-ahead}&\multicolumn{1}{c}{One-year-ahead}&\multicolumn{1}{c}{Two-year-ahead}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{ CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{ CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}\tabularnewline
\midrule
{\scshape S}&&&&&&&&&&&&&&&&&\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   0.984&   1.002&   0.989&   &   0.997&   \textbf{0.980 (1)}&   0.975&   &   1.011&   0.986&   1.023&   &   0.979&   0.989&   1.002\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   0.971 (2)&   0.996&   0.981***&   &   0.986&   0.990 (3)&   0.917*&   &   1.008&   0.999&   0.971&   &   0.959**&   0.993&   0.984\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   \textbf{0.967 (1)}&   0.982&   0.986&   &   0.992&   1.000&   0.876**&   &   0.979&   0.987&   0.973&   &   0.982&   0.983&   1.000\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   0.976&   0.976&   0.971***&   &   0.997&   1.021&   0.867**&   &   0.976&   0.994&   0.940&   &   0.963*&   0.975*&   0.974\tabularnewline
\shadeRow   ~~&   SSVS&   &   1.003&   1.025*&   1.016**&   &   1.018&   0.984 (2)&   1.017&   &   1.044&   1.013&   1.026&   &   1.034**&   0.984&   1.061***\tabularnewline
\midrule
{\scshape FA}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.013&   1.031**&   1.008&   &   0.956&   1.052*&   1.018&   &   1.069**&   1.025&   0.994&   &   1.070*&   0.980&   0.983\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   0.997&   1.015&   0.999&   &   0.939&   1.038&   0.998&   &   1.036&   1.018&   0.982&   &   0.990&   0.996&   1.016\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   0.996&   1.012&   0.978**&   &   0.939&   1.062&   0.951&   &   1.068*&   0.990&   0.985&   &   0.973&   0.972* (3)&   0.997\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.010&   1.010&   0.982**&   &   0.943&   1.095&   0.946&   &   1.076&   \textbf{0.971 (1)}&   1.002&   &   0.964*&   0.992&   0.987\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   1.022&   0.997&   0.983&   &   0.937&   1.118&   0.959&   &   1.009&   0.992&   0.993&   &   0.952**&   0.994&   1.001\tabularnewline
\shadeRow   ~~&   SSVS&   &   1.284***&   1.275***&   1.263***&   &   0.922&   1.583***&   1.214**&   &   1.112***&   1.454***&   1.124*&   &   1.072**&   1.424***&   1.184***\tabularnewline
\midrule
{\scshape M}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.020&   0.998&   1.011&   &   0.881** (3)&   1.136*&   0.992&   &   1.020&   0.982&   1.003&   &   1.027&   0.993&   1.027\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   1.001&   0.968&   0.981&   &   0.868*** (2)&   1.145*&   0.911&   &   0.972&   0.977 (3)&   0.947&   &   0.976&   0.988&   0.972\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   0.974&   0.967&   0.958***&   &   \textbf{0.859*** (1)}&   1.138*&   0.830***&   &   0.965&   0.986&   0.934&   &   0.950&   0.979&   0.925***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   0.972 (3)&   0.954&   0.933***&   &   0.928**&   1.091&   0.814***&   &   0.958&   0.983&   0.889*&   &   0.931***&   \textbf{0.956*** (1)}&   0.887***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   0.988&   0.947*&   0.951***&   &   0.972&   1.091&   0.823***&   &   0.951&   0.984&   0.869**&   &   0.942**&   0.984&   0.893***\tabularnewline
\shadeRow   ~~&   SSVS&   &   1.339***&   1.315***&   1.356***&   &   0.980&   1.653***&   1.235***&   &   1.132***&   1.482***&   1.213**&   &   1.178*&   1.474***&   1.349**\tabularnewline
\midrule
{\scshape L ($\theta_1 = 0.025$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.001&   0.986&   0.983&   &   0.895**&   1.105&   0.950&   &   1.004&   0.981&   0.972&   &   0.999&   0.974**&   0.980\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   1.020&   0.955&   0.955***&   &   0.969&   1.134*&   0.882**&   &   0.966&   0.974 (2)&   0.903*&   &   0.945**&   0.979*&   0.916***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   1.034&   0.958&   0.955***&   &   0.993&   1.125&   0.922&   &   0.973&   0.983&   0.886**&   &   0.945*&   0.979&   0.920**\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.025&   0.957&   0.955***&   &   1.005&   1.103&   0.910&   &   0.959&   0.988&   0.894*&   &   0.925***&   0.988&   0.924***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   1.034&   0.963&   0.950***&   &   1.006&   1.117&   0.921&   &   0.969&   0.994&   0.891**&   &   0.935***&   0.973*&   0.922**\tabularnewline
\midrule
{\scshape L ($\theta_1 = 0.050$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.003&   0.994&   0.989&   &   0.922&   1.081&   0.966&   &   1.026&   0.980&   0.982&   &   1.009&   0.984&   0.972\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   0.985&   0.948*&   0.938***&   &   0.903***&   1.128&   0.834***&   &   0.955&   0.984&   0.865**&   &   0.936***&   0.969* (2)&   0.874***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   1.015&   0.940**&   0.933***&   &   0.970&   1.140*&   0.849**&   &   0.949&   0.989&   0.828***&   &   0.926**&   0.985&   0.830***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.002&   0.940**&   0.932***&   &   0.980&   1.108&   0.840**&   &   0.947&   0.995&   0.820***&   &   0.924**&   0.980&   0.842***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   1.005&   0.939**&   0.932***&   &   0.980&   1.115&   0.840**&   &   0.944 (2)&   0.994&   0.821***&   &   0.925**&   0.978*&   0.844***\tabularnewline
\midrule
{\scshape L ($\theta_1 = 0.075$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.017&   1.001&   1.024&   &   0.943&   1.085&   0.989&   &   1.020&   0.988&   1.000&   &   1.073*&   0.993&   1.022\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   0.995&   0.935***&   0.934***&   &   0.905**&   1.146*&   0.841***&   &   0.944** (3)&   0.980&   0.833***&   &   0.923*** (3)&   0.980&   0.854***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   0.993&   0.930** (2)&   0.928*** (3)&   &   0.965&   1.133*&   0.780*** (2)&   &   0.948&   0.992&   0.778*** (3)&   &   0.915** (2)&   0.993&   0.809*** (3)\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.003&   \textbf{0.920** (1)}&   0.926*** (2)&   &   1.016&   1.114&   0.790*** (3)&   &   \textbf{0.930 (1)}&   0.991&   \textbf{0.762*** (1)}&   &   0.928*&   0.998&   \textbf{0.771*** (1)}\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   0.995&   0.930** (3)&   \textbf{0.925*** (1)}&   &   0.987&   1.122&   \textbf{0.780*** (1)}&   &   0.956&   0.989&   0.778*** (2)&   &   \textbf{0.909*** (1)}&   1.000&   0.791*** (2)\tabularnewline
\bottomrule
\end{tabular}}
\caption{CRPS ratios relative to the \textit{small-scale} BVAR with a Minnesota prior. \label{tab:CRPS}}
\begin{minipage}{\linewidth}
\footnotesize \textbf{Notes}: Bold numbers indicate lowest CRPS ratios for each horizon and target variable (and therefore best performing models over the full hold-out sample in terms of density forecasts), while the numbers in parenthesis refer to the ranking of the three best specifications. Gray shaded rows denote non-sparsified models. Asterisks indicate statistical significance for each model relative to the benchmark at the $1$ ($^{***}$), $5$ ($^{**}$) and $10$ ($^{*}$) percent significance levels. 
\end{minipage}\end{center}}
\end{table}

==> CRPS_full.tex <==
%latex.default(lps.all, file = paste0(score.type, "_", eval.type,     ".tex"), title = "", ctable = FALSE, rgroupTexCmd = "scshape",     n.cgroup = n.cgroup, cgroup = cgroup, colheads = colheads,     rgroup = rgroup, n.rgroup = n.rgroup, caption = "", label = "tab:dens",     size = "tiny", rownamesTexCmd = my.rownamesTexCmd, booktabs = TRUE,     rowname = "", numeric.dollar = FALSE, caption.loc = "bottom",     landscape = TRUE)%
\begin{landscape}\begin{table}[!tbp]
{\tiny
\begin{center}
\scalebox{0.9}{
\begin{tabular}{llclllclllclllclll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{1}{c}{\bfseries Spec.}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Avg.}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal 1-step-ahead}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal 4-step-ahead}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal 8-step-ahead}\tabularnewline
\cline{2-2} \cline{4-6} \cline{8-10} \cline{12-14} \cline{16-18}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{1-step ahead}&\multicolumn{1}{c}{4-step ahead}&\multicolumn{1}{c}{8-step ahead}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{ CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{ CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}\tabularnewline
\midrule
{\scshape Small}&&&&&&&&&&&&&&&&&\tabularnewline
   ~~&   MIN - $\lambda = 0.005$&   &   1.002&   1.004&   0.988&   &   1.010&   0.990&   1.013&   &   1.022&   0.996&   0.998&   &   0.983&   0.980&   1.011\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   0.984&   1.002&   0.989&   &   0.997&   0.980&   0.975&   &   1.011&   0.986&   1.023&   &   0.979&   0.989&   1.002\tabularnewline
   ~~&   MIN - $\lambda = 0.05$&   &   0.983&   0.996&   0.983&   &   1.016&   \textbf{0.973}&   0.958&   &   1.012&   0.989&   0.989&   &   0.980&   0.980***&   0.993\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   0.971&   0.996&   0.981***&   &   0.986&   0.990&   0.917*&   &   1.008&   0.999&   0.971&   &   0.959**&   0.993&   0.984\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   0.967&   0.982&   0.986&   &   0.992&   1.000&   0.876**&   &   0.979&   0.987&   0.973&   &   0.982&   0.983&   1.000\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   0.976&   0.976&   0.971***&   &   0.997&   1.021&   0.867**&   &   0.976&   0.994&   0.940&   &   0.963*&   0.975*&   0.974\tabularnewline
\shadeRow   ~~&   SSVS&   &   1.003&   1.025*&   1.016**&   &   1.018&   0.984&   1.017&   &   1.044&   1.013&   1.026&   &   1.034**&   0.984&   1.061***\tabularnewline
\midrule
{\scshape FAVAR}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.013&   1.031**&   1.008&   &   0.956&   1.052*&   1.018&   &   1.069**&   1.025&   0.994&   &   1.070*&   0.980&   0.983\tabularnewline
   ~~&   MIN - $\lambda = 0.005$&   &   0.994&   1.015&   1.003&   &   0.933&   1.038&   0.995&   &   1.076***&   1.000&   0.968&   &   1.014&   0.985&   1.027\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   0.997&   1.015&   0.999&   &   0.939&   1.038&   0.998&   &   1.036&   1.018&   0.982&   &   0.990&   0.996&   1.016\tabularnewline
   ~~&   MIN - $\lambda = 0.05$&   &   1.001&   1.017&   0.992&   &   0.952&   1.036&   1.000&   &   1.078**&   0.989&   0.994&   &   0.999&   0.988&   0.993\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   0.996&   1.012&   0.978**&   &   0.939&   1.062&   0.951&   &   1.068*&   0.990&   0.985&   &   0.973&   0.972*&   0.997\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.010&   1.010&   0.982**&   &   0.943&   1.095&   0.946&   &   1.076&   \textbf{0.971}&   1.002&   &   0.964*&   0.992&   0.987\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   1.022&   0.997&   0.983&   &   0.937&   1.118&   0.959&   &   1.009&   0.992&   0.993&   &   0.952**&   0.994&   1.001\tabularnewline
\shadeRow   ~~&   SSVS&   &   1.284***&   1.275***&   1.263***&   &   0.922&   1.583***&   1.214**&   &   1.112***&   1.454***&   1.124*&   &   1.072**&   1.424***&   1.184***\tabularnewline
\midrule
{\scshape Medium}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.020&   0.998&   1.011&   &   0.881**&   1.136*&   0.992&   &   1.020&   0.982&   1.003&   &   1.027&   0.993&   1.027\tabularnewline
   ~~&   MIN - $\lambda = 0.005$&   &   1.000&   0.992&   0.986&   &   \textbf{0.850***}&   1.146*&   0.933&   &   1.007&   0.991&   0.975&   &   0.971&   0.986&   1.006\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   1.001&   0.968&   0.981&   &   0.868***&   1.145*&   0.911&   &   0.972&   0.977&   0.947&   &   0.976&   0.988&   0.972\tabularnewline
   ~~&   MIN - $\lambda = 0.05$&   &   \textbf{0.966}&   0.963&   0.961***&   &   0.850***&   1.121&   0.839***&   &   0.978&   0.985&   0.901***&   &   0.950**&   0.980&   0.937***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   0.974&   0.967&   0.958***&   &   0.859***&   1.138*&   0.830***&   &   0.965&   0.986&   0.934&   &   0.950&   0.979&   0.925***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   0.972&   0.954&   0.933***&   &   0.928**&   1.091&   0.814***&   &   0.958&   0.983&   0.889*&   &   0.931***&   \textbf{0.956***}&   0.887***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   0.988&   0.947*&   0.951***&   &   0.972&   1.091&   0.823***&   &   0.951&   0.984&   0.869**&   &   0.942**&   0.984&   0.893***\tabularnewline
\shadeRow   ~~&   SSVS&   &   1.339***&   1.315***&   1.356***&   &   0.980&   1.653***&   1.235***&   &   1.132***&   1.482***&   1.213**&   &   1.178*&   1.474***&   1.349**\tabularnewline
\midrule
{\scshape Large ($\theta_1 = 0.025$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.001&   0.986&   0.983&   &   0.895**&   1.105&   0.950&   &   1.004&   0.981&   0.972&   &   0.999&   0.974**&   0.980\tabularnewline
   ~~&   MIN - $\lambda = 0.005$&   &   1.003&   0.961&   0.955***&   &   0.944**&   1.123&   0.864**&   &   0.965&   0.977&   0.922*&   &   0.964&   0.968*&   0.915***\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   1.020&   0.955&   0.955***&   &   0.969&   1.134*&   0.882**&   &   0.966&   0.974&   0.903*&   &   0.945**&   0.979*&   0.916***\tabularnewline
   ~~&   MIN - $\lambda = 0.05$&   &   1.026&   0.953*&   0.963**&   &   1.001&   1.111&   0.904&   &   0.951*&   0.981&   0.899**&   &   0.956&   0.985&   0.924**\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   1.034&   0.958&   0.955***&   &   0.993&   1.125&   0.922&   &   0.973&   0.983&   0.886**&   &   0.945*&   0.979&   0.920**\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.025&   0.957&   0.955***&   &   1.005&   1.103&   0.910&   &   0.959&   0.988&   0.894*&   &   0.925***&   0.988&   0.924***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   1.034&   0.963&   0.950***&   &   1.006&   1.117&   0.921&   &   0.969&   0.994&   0.891**&   &   0.935***&   0.973*&   0.922**\tabularnewline
\midrule
{\scshape Large ($\theta_1 = 0.050$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.003&   0.994&   0.989&   &   0.922&   1.081&   0.966&   &   1.026&   0.980&   0.982&   &   1.009&   0.984&   0.972\tabularnewline
   ~~&   MIN - $\lambda = 0.005$&   &   0.981&   0.949**&   0.948***&   &   0.898***&   1.111&   0.856***&   &   0.959&   0.980&   0.871***&   &   0.937***&   0.980&   0.895***\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   0.985&   0.948*&   0.938***&   &   0.903***&   1.128&   0.834***&   &   0.955&   0.984&   0.865**&   &   0.936***&   0.969*&   0.874***\tabularnewline
   ~~&   MIN - $\lambda = 0.05$&   &   0.997&   0.942*&   0.943***&   &   0.961&   1.122&   0.822***&   &   0.945&   0.989&   0.841***&   &   0.922***&   0.996&   0.858***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   1.015&   0.940**&   0.933***&   &   0.970&   1.140*&   0.849**&   &   0.949&   0.989&   0.828***&   &   0.926**&   0.985&   0.830***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.002&   0.940**&   0.932***&   &   0.980&   1.108&   0.840**&   &   0.947&   0.995&   0.820***&   &   0.924**&   0.980&   0.842***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   1.005&   0.939**&   0.932***&   &   0.980&   1.115&   0.840**&   &   0.944&   0.994&   0.821***&   &   0.925**&   0.978*&   0.844***\tabularnewline
\midrule
{\scshape Large ($\theta_1 = 0.075$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.017&   1.001&   1.024&   &   0.943&   1.085&   0.989&   &   1.020&   0.988&   1.000&   &   1.073*&   0.993&   1.022\tabularnewline
   ~~&   MIN - $\lambda = 0.005$&   &   1.004&   0.952**&   0.938***&   &   0.911*&   1.135&   0.887*&   &   0.942**&   1.007&   0.852***&   &   0.929***&   0.982&   0.859***\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   0.995&   0.935***&   0.934***&   &   0.905**&   1.146*&   0.841***&   &   0.944**&   0.980&   0.833***&   &   0.923***&   0.980&   0.854***\tabularnewline
   ~~&   MIN - $\lambda = 0.05$&   &   0.973&   0.930**&   0.926***&   &   0.929**&   1.114&   \textbf{0.779***}&   &   0.942&   0.988&   0.795***&   &   0.928**&   0.977&   0.814***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   0.993&   0.930**&   0.928***&   &   0.965&   1.133*&   0.780***&   &   0.948&   0.992&   0.778***&   &   0.915**&   0.993&   0.809***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.003&   \textbf{0.920**}&   0.926***&   &   1.016&   1.114&   0.790***&   &   \textbf{0.930}&   0.991&   \textbf{0.762***}&   &   0.928*&   0.998&   \textbf{0.771***}\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   0.995&   0.930**&   \textbf{0.925***}&   &   0.987&   1.122&   0.780***&   &   0.956&   0.989&   0.778***&   &   \textbf{0.909***}&   1.000&   0.791***\tabularnewline
\bottomrule
\end{tabular}}
\caption{CRPS ratios relative to the \textit{small-scale} BVAR with a Minnesota prior. \label{tab:CRPS}}
\begin{minipage}{\linewidth}
\footnotesize \textbf{Notes}: Bold numbers indicate lowest CRPS ratios for each horizon and target variable (and therefore best performing models over the full hold-out sample in terms of density forecasts). Gray shaded rows denote non-sparsified models. Asterisks indicate statistical significance for each model relative to the benchmark at the $1$ ($^{***}$), $5$ ($^{**}$) and $10$ ($^{*}$) percent significance levels. 
\end{minipage}\end{center}}
\end{table}\end{landscape}


==> LPS_final.tex <==
%latex.default(lps.all, file = paste0(score.type, "_", eval.type,     ".tex"), title = "", ctable = FALSE, rgroupTexCmd = "scshape",     n.cgroup = n.cgroup, cgroup = cgroup, colheads = colheads,     rgroup = rgroup, n.rgroup = n.rgroup, caption = "", label = "tab:dens",     size = "tiny", rownamesTexCmd = my.rownamesTexCmd, booktabs = TRUE,     rowname = "", numeric.dollar = FALSE, caption.loc = "bottom",     landscape = TRUE)%
\begin{landscape}\begin{table}[!tbp]
{\tiny
\begin{center}
\scalebox{0.95}{
\begin{tabular}{llclllclllclllclll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{1}{c}{\bfseries Spec.}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Joint}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal 1-step-ahead}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal 4-step-ahead}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal 8-step-ahead}\tabularnewline
\cline{2-2} \cline{4-6} \cline{8-10} \cline{12-14} \cline{16-18}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{1-step ahead}&\multicolumn{1}{c}{4-step ahead}&\multicolumn{1}{c}{8-step ahead}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{ CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{ CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}\tabularnewline
\midrule
{\scshape Small}&&&&&&&&&&&&&&&&&\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &     5.745**&     4.828*&     4.513&   &    0.634&     0.897&    3.187***&   &    1.570&     0.011&    1.697*&   &     2.596***&    -1.680&     2.722***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &     7.534&     7.745*&     6.118&   &    0.212&     0.198&    6.525**&   &    2.945&    -0.850&    3.558*&   &     4.365***&    -3.968&     5.467***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &     6.817&     9.475&     5.437&   &    0.526&    -2.596&    9.088***&   &    4.457*&    -1.418&    6.169***&   &     5.880***&    -7.634&     8.116***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &     5.288&    10.737&     5.783&   &    1.515&    -4.985&    9.801***&   &    5.147*&    -1.903&    7.587***&   &     6.561***&    -8.251&     9.464***\tabularnewline
\shadeRow   ~~&   SSVS&   &    -3.705&    -0.176&    -4.098&   &   -3.035***&     4.484&   -2.205&   &   -4.165***&   \textbf{  6.517}&   -2.751***&   &    -3.609***&   \textbf{  4.654}&    -4.478***\tabularnewline
\midrule
{\scshape FAVAR}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &    17.948&     2.769&    -3.098&   &   11.408**&     4.423&    6.088&   &   -1.815&     0.329&    1.871***&   &    -3.025&    -0.454&     0.819\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &    19.086&     5.844&     2.745&   &   11.634**&   \textbf{  4.606}&    7.538&   &   -0.776&     1.619&    2.700***&   &     1.460&    -2.279&     2.561***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &    17.368&     5.394&     4.983&   &   11.687**&     1.624&    9.088&   &   -1.320&     0.361&    2.997*&   &     4.656***&    -5.399&     4.700***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &    10.393&     6.816&     7.252&   &   11.893**&    -5.325&   11.055*&   &    0.072&    -1.207&    3.496*&   &     6.809***&    -3.661&     6.073***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &     5.528&    10.154*&     8.667&   &   12.101**&    -7.035&   11.863**&   &    1.778&    -1.433&    4.315**&   &     7.417**&    -3.304&     6.539***\tabularnewline
\shadeRow   ~~&   SSVS&   &   -46.196&   -28.238&   -35.739&   &    9.724&   -51.723*&   -6.802&   &   -5.828**&   -30.101&   -6.738**&   &    -5.940***&   -31.360&   -10.958***\tabularnewline
\midrule
{\scshape Medium}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &    20.032&     7.907&    -1.659***&   &   17.376**&    -2.255&    6.753**&   &    0.828&     5.649&   -0.515&   &    -0.931*&     0.515&    -0.295\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &    26.850&    12.099**&     8.382&   &   \textbf{20.002***}&    -3.443&   12.838***&   &    5.318**&     0.214&    6.416***&   &     6.115**&    -4.446&     8.134***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   \textbf{ 30.006**}&    23.425***&    13.825&   &   19.219***&    -6.633&   18.867***&   &    8.621&    -3.174&   14.480***&   &     9.698*&   -10.551&    16.545***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &    16.531&    22.625&   \textbf{ 18.330}&   &   11.862***&   -13.195&   20.096***&   &   10.468&    -6.613&   21.016***&   &    11.235&   -15.732&    22.923***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &    10.911&   \textbf{ 23.489}&    17.980&   &    6.597*&   -15.470&   19.296***&   &   10.689&    -8.354&   22.812***&   &    11.501&   -18.285&    24.700***\tabularnewline
\shadeRow   ~~&   SSVS&   &   -68.116&   -50.493*&   -67.513*&   &    2.288&   -68.574*&   -3.879&   &   -9.995**&   -40.090&   -7.634&   &   -17.749**&   -37.498&   -19.086**\tabularnewline
\midrule
{\scshape Large ($\theta_1 = 0.025$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &     7.597&     8.680&     1.966&   &   10.798**&    -4.707&    3.624&   &    4.307*&     0.243&    3.658***&   &     2.764*&    -4.571&     5.158***\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &    -1.374&    16.156&    14.614&   &    5.550**&   -15.415&    9.195***&   &    9.270*&    -8.006&   14.482***&   &    10.447*&   -11.916&    16.407***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &    -8.248&    16.134&    15.324&   &    0.544&   -17.598&    8.403**&   &    9.459&    -9.092&   15.961***&   &    10.729*&   -13.387&    17.765***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &    -6.784&    16.336&    15.528&   &    0.900&   -17.445&    8.692**&   &    9.528&    -9.174&   16.198***&   &    10.796*&   -13.520&    17.978***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &    -6.225&    16.389&    15.621&   &    1.002&   -17.345&    8.827**&   &    9.537&    -9.180&   16.253***&   &    10.807*&   -13.522&    18.028***\tabularnewline
\midrule
{\scshape Large ($\theta_1 = 0.050$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &     6.284&     5.536&    -0.471&   &   11.666**&    -8.084&    6.990*&   &    3.225&     0.217&    2.864***&   &    -0.132&    -1.901&     4.406***\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &     8.616&    14.644&     9.218&   &   13.873***&   -19.797*&   19.791***&   &   11.511&   -18.799&   23.511***&   &    12.242&   -24.021&    25.737***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &    -8.814&     1.967&     1.320&   &    4.464&   -33.086**&   22.504***&   &   10.734&   -34.528&   30.543***&   &    12.070&   -37.301&    32.828***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   -14.061&     2.130&    -0.703&   &    1.067&   -38.927*&   22.677***&   &   10.718&   -38.134&   31.721***&   &    12.100&   -39.940&    33.905***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   -12.870&     2.495&    -0.578&   &    1.209&   -39.186*&   23.364***&   &   10.841&   -38.322&   31.969***&   &    12.144&   -40.097&    34.082***\tabularnewline
\midrule
{\scshape Large ($\theta_1 = 0.075$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &     6.470&     2.303&    -5.543&   &   11.749*&    -9.162&   11.388***&   &    2.937&     0.124&    0.444&   &    -2.815&    -2.295&     1.106\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &    -1.536&     8.305&     6.836&   &   17.102***&   -28.712*&   24.434***&   &   \textbf{12.856*}&   -30.720&   28.291***&   &   \textbf{ 12.898}&   -31.633&    31.334***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &    -4.866&   -20.495&   -22.643&   &    9.246**&   -40.233**&   31.976***&   &    8.744&   -66.632&   39.748***&   &    10.139&   -69.578&    42.767***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   -42.144&   -30.466&   -30.732&   &   -1.292&   -69.624*&   31.766***&   &    7.426&   -76.417&   42.522***&   &     8.980&   -83.052&    45.338***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   -46.109&   -30.932&   -31.000&   &   -2.662&   -71.845*&   \textbf{32.671***}&   &    7.565&   -77.508&   \textbf{43.035***}&   &     8.984&   -84.153&   \textbf{ 45.706***}\tabularnewline
\bottomrule
\end{tabular}}
\caption{Bayes factors relative to the \textit{small-scale} BVAR with a Minnesota prior. \label{tab:LPS}}
\begin{minipage}{\linewidth}
\footnotesize \textbf{Notes}: Bold numbers indicate highest Bayes factors for each horizon and target variable (and therefore best performing models over the full hold-out sample in terms of density forecasts). Gray shaded rows denote non-sparsified models. Asterisks indicate statistical significance for each model relative to the benchmark at the $1$ ($^{***}$), $5$ ($^{**}$) and $10$ ($^{*}$) percent significance levels. 
\end{minipage}\end{center}}
\end{table}\end{landscape}


==> LPS_full.tex <==
%latex.default(lps.all, file = paste0(score.type, "_", eval.type,     ".tex"), title = "", ctable = FALSE, rgroupTexCmd = "scshape",     n.cgroup = n.cgroup, cgroup = cgroup, colheads = colheads,     rgroup = rgroup, n.rgroup = n.rgroup, caption = "", label = "tab:dens",     size = "tiny", rownamesTexCmd = my.rownamesTexCmd, booktabs = TRUE,     rowname = "", numeric.dollar = FALSE, caption.loc = "bottom",     landscape = TRUE)%
\begin{landscape}\begin{table}[!tbp]
{\tiny
\begin{center}
\scalebox{0.9}{
\begin{tabular}{llclllclllclllclll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{1}{c}{\bfseries Spec.}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Joint}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal 1-step-ahead}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal 4-step-ahead}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal 8-step-ahead}\tabularnewline
\cline{2-2} \cline{4-6} \cline{8-10} \cline{12-14} \cline{16-18}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{1-step ahead}&\multicolumn{1}{c}{4-step ahead}&\multicolumn{1}{c}{8-step ahead}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{ CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{ CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}\tabularnewline
\midrule
{\scshape Small}&&&&&&&&&&&&&&&&&\tabularnewline
   ~~&   MIN - $\lambda = 0.005$&   &     4.252**&     3.653&     3.705*&   &    0.539&     0.692&    2.291***&   &    1.139*&     0.036&    1.218*&   &     1.958***&    -1.523&     1.957***\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &     5.745**&     4.828*&     4.513&   &    0.634&     0.897&    3.187***&   &    1.570&     0.011&    1.697*&   &     2.596***&    -1.680&     2.722***\tabularnewline
   ~~&   MIN - $\lambda = 0.05$&   &     7.333*&     7.044*&     6.101&   &    0.433&     0.860&    5.414**&   &    2.491&    -0.455&    2.924*&   &     3.896***&    -2.853&     4.667***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &     7.534&     7.745*&     6.118&   &    0.212&     0.198&    6.525**&   &    2.945&    -0.850&    3.558*&   &     4.365***&    -3.968&     5.467***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &     6.817&     9.475&     5.437&   &    0.526&    -2.596&    9.088***&   &    4.457*&    -1.418&    6.169***&   &     5.880***&    -7.634&     8.116***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &     5.288&    10.737&     5.783&   &    1.515&    -4.985&    9.801***&   &    5.147*&    -1.903&    7.587***&   &     6.561***&    -8.251&     9.464***\tabularnewline
\shadeRow   ~~&   SSVS&   &    -3.705&    -0.176&    -4.098&   &   -3.035***&     4.484&   -2.205&   &   -4.165***&   \textbf{  6.517}&   -2.751***&   &    -3.609***&   \textbf{  4.654}&    -4.478***\tabularnewline
\midrule
{\scshape FAVAR}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &    17.948&     2.769&    -3.098&   &   11.408**&     4.423&    6.088&   &   -1.815&     0.329&    1.871***&   &    -3.025&    -0.454&     0.819\tabularnewline
   ~~&   MIN - $\lambda = 0.005$&   &    18.633&     6.183&     1.928&   &   11.778**&   \textbf{  4.888}&    7.455&   &   -0.706&     1.872&    2.583***&   &     0.555&    -1.386&     2.155***\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &    19.086&     5.844&     2.745&   &   11.634**&     4.606&    7.538&   &   -0.776&     1.619&    2.700***&   &     1.460&    -2.279&     2.561***\tabularnewline
   ~~&   MIN - $\lambda = 0.05$&   &    19.344&     6.363&     3.779&   &   11.578**&     3.590&    8.418&   &   -1.267&     0.657&    2.883**&   &     3.698***&    -4.917&     3.975***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &    17.368&     5.394&     4.983&   &   11.687**&     1.624&    9.088&   &   -1.320&     0.361&    2.997*&   &     4.656***&    -5.399&     4.700***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &    10.393&     6.816&     7.252&   &   11.893**&    -5.325&   11.055*&   &    0.072&    -1.207&    3.496*&   &     6.809***&    -3.661&     6.073***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &     5.528&    10.154*&     8.667&   &   12.101**&    -7.035&   11.863**&   &    1.778&    -1.433&    4.315**&   &     7.417**&    -3.304&     6.539***\tabularnewline
\shadeRow   ~~&   SSVS&   &   -46.196&   -28.238&   -35.739&   &    9.724&   -51.723*&   -6.802&   &   -5.828**&   -30.101&   -6.738**&   &    -5.940***&   -31.360&   -10.958***\tabularnewline
\midrule
{\scshape Medium}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &    20.032&     7.907&    -1.659***&   &   17.376**&    -2.255&    6.753**&   &    0.828&     5.649&   -0.515&   &    -0.931*&     0.515&    -0.295\tabularnewline
   ~~&   MIN - $\lambda = 0.005$&   &    23.855&    11.048**&     6.547&   &   19.449***&    -2.955&   11.142***&   &    4.403***&     1.343&    4.939***&   &     4.917**&    -3.670&     6.377***\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &    26.850&    12.099**&     8.382&   &   20.002***&    -3.443&   12.838***&   &    5.318**&     0.214&    6.416***&   &     6.115**&    -4.446&     8.134***\tabularnewline
   ~~&   MIN - $\lambda = 0.05$&   &    29.748*&    19.413***&    12.626&   &   \textbf{20.199***}&    -7.442&   17.152***&   &    7.533*&    -2.189&   11.551***&   &     8.749**&    -7.690&    13.629***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   \textbf{ 30.006**}&    23.425***&    13.825&   &   19.219***&    -6.633&   18.867***&   &    8.621&    -3.174&   14.480***&   &     9.698*&   -10.551&    16.545***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &    16.531&    22.625&   \textbf{ 18.330}&   &   11.862***&   -13.195&   20.096***&   &   10.468&    -6.613&   21.016***&   &    11.235&   -15.732&    22.923***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &    10.911&   \textbf{ 23.489}&    17.980&   &    6.597*&   -15.470&   19.296***&   &   10.689&    -8.354&   22.812***&   &    11.501&   -18.285&    24.700***\tabularnewline
\shadeRow   ~~&   SSVS&   &   -68.116&   -50.493*&   -67.513*&   &    2.288&   -68.574*&   -3.879&   &   -9.995**&   -40.090&   -7.634&   &   -17.749**&   -37.498&   -19.086**\tabularnewline
\midrule
{\scshape Large ($\theta_1 = 0.025$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &     7.597&     8.680&     1.966&   &   10.798**&    -4.707&    3.624&   &    4.307*&     0.243&    3.658***&   &     2.764*&    -4.571&     5.158***\tabularnewline
   ~~&   MIN - $\lambda = 0.005$&   &     1.643&    16.187&    14.072&   &    7.680***&   -14.316&    9.091***&   &    9.131*&    -7.062&   13.357***&   &    10.190**&   -10.943&    15.283***\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &    -1.374&    16.156&    14.614&   &    5.550**&   -15.415&    9.195***&   &    9.270*&    -8.006&   14.482***&   &    10.447*&   -11.916&    16.407***\tabularnewline
   ~~&   MIN - $\lambda = 0.05$&   &    -8.038&    16.100&    15.246&   &    1.158&   -17.145&    8.543**&   &    9.418&    -8.949&   15.780***&   &    10.682*&   -13.199&    17.604***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &    -8.248&    16.134&    15.324&   &    0.544&   -17.598&    8.403**&   &    9.459&    -9.092&   15.961***&   &    10.729*&   -13.387&    17.765***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &    -6.784&    16.336&    15.528&   &    0.900&   -17.445&    8.692**&   &    9.528&    -9.174&   16.198***&   &    10.796*&   -13.520&    17.978***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &    -6.225&    16.389&    15.621&   &    1.002&   -17.345&    8.827**&   &    9.537&    -9.180&   16.253***&   &    10.807*&   -13.522&    18.028***\tabularnewline
\midrule
{\scshape Large ($\theta_1 = 0.050$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &     6.284&     5.536&    -0.471&   &   11.666**&    -8.084&    6.990*&   &    3.225&     0.217&    2.864***&   &    -0.132&    -1.901&     4.406***\tabularnewline
   ~~&   MIN - $\lambda = 0.005$&   &    10.152&    17.854&    10.953&   &   14.879***&   -18.464&   17.790***&   &   11.514**&   -14.338&   20.578***&   &    11.983*&   -19.196&    22.647***\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &     8.616&    14.644&     9.218&   &   13.873***&   -19.797*&   19.791***&   &   11.511&   -18.799&   23.511***&   &    12.242&   -24.021&    25.737***\tabularnewline
   ~~&   MIN - $\lambda = 0.05$&   &    -4.275&     4.120&     4.362&   &    8.137**&   -29.570**&   22.536***&   &   10.876&   -29.931&   29.184***&   &    12.116&   -34.364&    31.525***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &    -8.814&     1.967&     1.320&   &    4.464&   -33.086**&   22.504***&   &   10.734&   -34.528&   30.543***&   &    12.070&   -37.301&    32.828***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   -14.061&     2.130&    -0.703&   &    1.067&   -38.927*&   22.677***&   &   10.718&   -38.134&   31.721***&   &    12.100&   -39.940&    33.905***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   -12.870&     2.495&    -0.578&   &    1.209&   -39.186*&   23.364***&   &   10.841&   -38.322&   31.969***&   &    12.144&   -40.097&    34.082***\tabularnewline
\midrule
{\scshape Large ($\theta_1 = 0.075$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &     6.470&     2.303&    -5.543&   &   11.749*&    -9.162&   11.388***&   &    2.937&     0.124&    0.444&   &    -2.815&    -2.295&     1.106\tabularnewline
   ~~&   MIN - $\lambda = 0.005$&   &    -1.291&    12.561&    10.142&   &   17.056***&   -25.371&   22.278***&   &   12.582**&   -22.582&   24.148***&   &   \textbf{ 12.904*}&   -25.145&    27.189***\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &    -1.536&     8.305&     6.836&   &   17.102***&   -28.712*&   24.434***&   &   \textbf{12.856*}&   -30.720&   28.291***&   &    12.898&   -31.633&    31.334***\tabularnewline
   ~~&   MIN - $\lambda = 0.05$&   &    -0.699&    -9.468&   -13.712&   &   13.051***&   -35.139**&   31.137***&   &   10.362&   -56.067&   37.049***&   &    11.068&   -55.741&    40.202***\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &    -4.866&   -20.495&   -22.643&   &    9.246**&   -40.233**&   31.976***&   &    8.744&   -66.632&   39.748***&   &    10.139&   -69.578&    42.767***\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   -42.144&   -30.466&   -30.732&   &   -1.292&   -69.624*&   31.766***&   &    7.426&   -76.417&   42.522***&   &     8.980&   -83.052&    45.338***\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   -46.109&   -30.932&   -31.000&   &   -2.662&   -71.845*&   \textbf{32.671***}&   &    7.565&   -77.508&   \textbf{43.035***}&   &     8.984&   -84.153&   \textbf{ 45.706***}\tabularnewline
\bottomrule
\end{tabular}}
\caption{Bayes factors relative to the \textit{small-scale} BVAR with a Minnesota prior. \label{tab:LPS}}
\begin{minipage}{\linewidth}
\footnotesize \textbf{Notes}: Bold numbers indicate highest Bayes factors for each horizon and target variable (and therefore best performing models over the full hold-out sample in terms of density forecasts). Gray shaded rows denote non-sparsified models. Asterisks indicate statistical significance for each model relative to the benchmark at the $1$ ($^{***}$), $5$ ($^{**}$) and $10$ ($^{*}$) percent significance levels. 
\end{minipage}\end{center}}
\end{table}\end{landscape}


==> MAD_AS_05.tex <==
%latex.default(MAD.AS.full, file = paste0("MAD_AS_", gsub(scale.v.mat.grid,     pattern = "\\.", replacement = ""), ".tex"), title = "",     ctable = FALSE, rgroupTexCmd = "scshape", n.cgroup = n.cgroup,     cgroup = cgroup, colheads = colheads, rgroup = rgroup, n.rgroup = n.rgroup,     caption = "", label = "tab:MAD-AS", size = "tiny", booktabs = TRUE,     numeric.dollar = TRUE, rowname = "", caption.loc = "bottom")%
\begin{table}[!tbp]
{\tiny
\begin{center}
\begin{tabular}{llllclllllcll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{3}{c}{\bfseries DGP}&\multicolumn{1}{c}{\bfseries }&\multicolumn{5}{c}{\bfseries Specification}&\multicolumn{1}{c}{\bfseries }&\multicolumn{2}{c}{\bfseries Alternatives with MIN - $\lambda = 1$}\tabularnewline
\cline{2-4} \cline{6-10} \cline{12-13}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{M}&\multicolumn{1}{c}{T}&\multicolumn{1}{c}{Sparsity}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{MIN - $\lambda = 0.01$}&\multicolumn{1}{c}{MIN - $\lambda = 0.1 $}&\multicolumn{1}{c}{MIN - $\lambda = 0.5 $}&\multicolumn{1}{c}{MIN - $\lambda = 1 $}&\multicolumn{1}{c}{SSVS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{SAVS - Median}&\multicolumn{1}{c}{CDA}\tabularnewline
\midrule
{\scshape COEFFICIENTS}&&&&&&&&&&&&\tabularnewline
~~&L&240&Dense&&\textbf{0.953}&1.005&1.070&1.086&1.075&&1.086&1.086\tabularnewline
~~&&&Moderate&&0.760&\textbf{0.735}&0.770&0.779&0.876&&0.779&0.779\tabularnewline
~~&&&Sparse&&0.577&0.441&\textbf{0.439}&0.442&0.704&&0.442&0.442\tabularnewline
~~&&80&Dense&&\textbf{0.984}&1.023&1.032&1.032&1.432&&1.032&1.032\tabularnewline
~~&&&Moderate&&0.800&\textbf{0.794}&0.798&0.798&1.513&&0.798&0.798\tabularnewline
~~&&&Sparse&&0.579&0.507&\textbf{0.507}&0.507&1.572&&0.507&0.507\tabularnewline
\midrule
{\scshape }&&&&&&&&&&&&\tabularnewline
~~&M&240&Dense&&\textbf{0.886}&0.890&0.927&0.960&0.963&&0.960&0.960\tabularnewline
~~&&&Moderate&&0.716&\textbf{0.642}&0.644&0.665&0.692&&0.665&0.665\tabularnewline
~~&&&Sparse&&0.588&0.423&\textbf{0.377}&0.382&0.505&&0.382&0.382\tabularnewline
~~&&80&Dense&&\textbf{0.913}&0.924&0.970&0.999&1.018&&0.999&0.999\tabularnewline
~~&&&Moderate&&0.758&0.697&\textbf{0.696}&0.710&0.797&&0.710&0.710\tabularnewline
~~&&&Sparse&&0.637&0.491&0.436&\textbf{0.436}&0.632&&0.436&0.436\tabularnewline
\midrule
{\scshape }&&&&&&&&&&&&\tabularnewline
~~&S&240&Dense&&0.844&\textbf{0.819}&0.846&0.865&0.865&&0.865&0.865\tabularnewline
~~&&&Moderate&&0.717&0.612&\textbf{0.604}&0.611&0.651&&0.611&0.611\tabularnewline
~~&&&Sparse&&0.618&0.454&0.414&\textbf{0.413}&0.505&&0.413&0.413\tabularnewline
~~&&80&Dense&&0.847&\textbf{0.818}&0.830&0.846&0.860&&0.846&0.846\tabularnewline
~~&&&Moderate&&0.727&0.636&\textbf{0.623}&0.629&0.669&&0.629&0.629\tabularnewline
~~&&&Sparse&&0.654&0.504&0.451&\textbf{0.446}&0.546&&0.446&0.446\tabularnewline
\midrule
{\scshape COVARIANCES}&&&&&&&&&&&&\tabularnewline
~~&L&240&Dense&&0.999&\textbf{0.993}&0.998&1.026&1.106&&1.026&1.026\tabularnewline
~~&&&Moderate&&0.996&0.966&0.887&0.841&\textbf{0.827}&&0.841&0.840\tabularnewline
~~&&&Sparse&&0.993&0.938&0.780&0.658&\textbf{0.604}&&0.658&0.656\tabularnewline
~~&&80&Dense&&0.999&0.992&0.968&\textbf{0.950}&1.004&&0.950&0.950\tabularnewline
~~&&&Moderate&&0.999&0.988&0.950&0.913&\textbf{0.809}&&0.913&0.912\tabularnewline
~~&&&Sparse&&0.998&0.985&0.934&0.882&\textbf{0.632}&&0.882&0.881\tabularnewline
\midrule
{\scshape }&&&&&&&&&&&&\tabularnewline
~~&M&240&Dense&&\textbf{1.000}&1.003&1.032&1.081&1.248&&1.081&1.082\tabularnewline
~~&&&Moderate&&0.996&0.973&0.915&0.889&\textbf{0.863}&&0.889&0.889\tabularnewline
~~&&&Sparse&&0.992&0.936&0.788&0.687&\textbf{0.639}&&0.687&0.686\tabularnewline
~~&&80&Dense&&1.000&\textbf{0.999}&1.000&1.007&1.174&&1.007&1.007\tabularnewline
~~&&&Moderate&&0.999&0.988&0.953&0.922&\textbf{0.826}&&0.922&0.922\tabularnewline
~~&&&Sparse&&0.998&0.980&0.918&0.859&\textbf{0.594}&&0.859&0.859\tabularnewline
\midrule
{\scshape }&&&&&&&&&&&&\tabularnewline
~~&S&240&Dense&&0.999&\textbf{0.999}&1.010&1.039&1.153&&1.039&1.039\tabularnewline
~~&&&Moderate&&0.994&0.955&0.871&0.835&\textbf{0.829}&&0.835&0.835\tabularnewline
~~&&&Sparse&&0.987&0.919&0.771&\textbf{0.694}&0.700&&0.694&0.694\tabularnewline
~~&&80&Dense&&1.000&\textbf{1.000}&1.001&1.007&1.090&&1.007&1.007\tabularnewline
~~&&&Moderate&&0.998&0.981&0.935&0.899&\textbf{0.792}&&0.899&0.899\tabularnewline
~~&&&Sparse&&0.996&0.971&0.903&0.847&\textbf{0.647}&&0.847&0.847\tabularnewline
\bottomrule
\end{tabular}
\caption{MAE ratios of coefficients and covariances to non-sparse BVAR estimates.\label{tab:MAD-A}} 
\begin{minipage}{\textwidth}
 \footnotesize\textbf{Notes:} Bold numbers indicate the smallest MAE ratio. We simulate a DGP for a \textit{small-scale} ($m = 3$), \textit{medium-scale} ($m = 10$) and \textit{large-scale} ($m = 30$) VAR for two different number of observations $T$ and for three different degrees of sparsity (zero parameters as percentage of total number of coefficients $k = m(mp + 1)$ and covariances $w = m(m + 1)/2$, ranging from a dense DGP to a fully sparse DGP. \texttt{SAVS-Med.} refers to a sparse estimator, where we minimize the expected loss of the posterior median \cite[see][]{hahncarvalho2015dss}, while for the \texttt{CDA} specification we replace the SAVS estimator with a coordinate descent algorithm, i.e. we do not stop after the first iteration for both coefficients and covariances. 
\end{minipage}\end{center}}
\end{table}


==> MAD_AS_4.tex <==
%latex.default(MAD.AS.full, file = paste0("MAD_AS_", gsub(scale.v.mat.grid,     pattern = "\\.", replacement = ""), ".tex"), title = "",     ctable = FALSE, rgroupTexCmd = "scshape", n.cgroup = n.cgroup,     cgroup = cgroup, colheads = colheads, rgroup = rgroup, n.rgroup = n.rgroup,     caption = "", label = "tab:MAD-AS", size = "tiny", booktabs = TRUE,     numeric.dollar = TRUE, rowname = "", caption.loc = "bottom")%
\begin{table}[!tbp]
{\tiny
\begin{center}
\begin{tabular}{llllclllllcll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{3}{c}{\bfseries DGP}&\multicolumn{1}{c}{\bfseries }&\multicolumn{5}{c}{\bfseries Specification}&\multicolumn{1}{c}{\bfseries }&\multicolumn{2}{c}{\bfseries Expected loss}\tabularnewline
\cline{2-4} \cline{6-10} \cline{12-13}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{M}&\multicolumn{1}{c}{T}&\multicolumn{1}{c}{Sparsity}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{MIN - $\lambda = 0.01$}&\multicolumn{1}{c}{MIN - $\lambda = 0.1 $}&\multicolumn{1}{c}{MIN - $\lambda = 0.5 $}&\multicolumn{1}{c}{MIN - $\lambda = 1 $}&\multicolumn{1}{c}{SSVS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{SAVS-Med.: MIN - $\lambda = 1 $}&\multicolumn{1}{c}{C.d.a.:  MIN - $\lambda = 1 $}\tabularnewline
\midrule
{\scshape COEFFICIENTS}&&&&&&&&&&&&\tabularnewline
~~&L&240&Dense&&\textbf{0.945}&0.956&0.996&1.025&1.107&&1.025&1.025\tabularnewline
~~&&&Moderate&&0.815&0.755&\textbf{0.736}&0.746&0.909&&0.746&0.746\tabularnewline
~~&&&Sparse&&0.713&0.574&0.478&\textbf{0.460}&0.751&&0.460&0.460\tabularnewline
~~&&80&Dense&&\textbf{0.970}&0.991&1.021&1.029&1.691&&1.029&1.029\tabularnewline
~~&&&Moderate&&0.851&0.806&\textbf{0.803}&0.806&1.838&&0.806&0.806\tabularnewline
~~&&&Sparse&&0.731&0.598&0.550&\textbf{0.547}&1.943&&0.547&0.547\tabularnewline
\midrule
{\scshape }&&&&&&&&&&&&\tabularnewline
~~&M&240&Dense&&0.904&\textbf{0.879}&0.886&0.897&0.972&&0.897&0.897\tabularnewline
~~&&&Moderate&&0.810&0.705&0.656&\textbf{0.648}&0.751&&0.648&0.648\tabularnewline
~~&&&Sparse&&0.751&0.583&0.475&\textbf{0.442}&0.602&&0.442&0.442\tabularnewline
~~&&80&Dense&&0.925&\textbf{0.913}&0.922&0.935&1.053&&0.935&0.935\tabularnewline
~~&&&Moderate&&0.833&0.760&0.720&\textbf{0.711}&0.844&&0.711&0.711\tabularnewline
~~&&&Sparse&&0.773&0.648&0.557&\textbf{0.524}&0.709&&0.524&0.524\tabularnewline
\midrule
{\scshape }&&&&&&&&&&&&\tabularnewline
~~&S&240&Dense&&0.911&0.845&\textbf{0.835}&0.841&0.888&&0.841&0.841\tabularnewline
~~&&&Moderate&&0.853&0.718&0.654&\textbf{0.644}&0.731&&0.644&0.644\tabularnewline
~~&&&Sparse&&0.820&0.641&0.541&\textbf{0.514}&0.652&&0.514&0.514\tabularnewline
~~&&80&Dense&&0.907&0.855&0.840&\textbf{0.839}&0.905&&0.839&0.839\tabularnewline
~~&&&Moderate&&0.856&0.747&0.692&\textbf{0.680}&0.763&&0.680&0.680\tabularnewline
~~&&&Sparse&&0.829&0.686&0.599&\textbf{0.572}&0.693&&0.572&0.572\tabularnewline
\midrule
{\scshape COVARIANCES}&&&&&&&&&&&&\tabularnewline
~~&L&240&Dense&&0.994&0.953&0.858&0.818&\textbf{0.806}&&0.818&0.818\tabularnewline
~~&&&Moderate&&0.992&0.938&0.791&0.693&\textbf{0.669}&&0.693&0.693\tabularnewline
~~&&&Sparse&&0.991&0.929&0.747&0.606&\textbf{0.570}&&0.606&0.605\tabularnewline
~~&&80&Dense&&0.998&0.984&0.934&0.885&\textbf{0.869}&&0.885&0.885\tabularnewline
~~&&&Moderate&&0.998&0.984&0.930&0.876&\textbf{0.782}&&0.876&0.875\tabularnewline
~~&&&Sparse&&0.998&0.983&0.928&0.871&\textbf{0.716}&&0.871&0.870\tabularnewline
\midrule
{\scshape }&&&&&&&&&&&&\tabularnewline
~~&M&240&Dense&&0.997&0.979&\textbf{0.958}&0.975&1.003&&0.975&0.975\tabularnewline
~~&&&Moderate&&0.993&0.945&0.835&0.778&\textbf{0.771}&&0.778&0.777\tabularnewline
~~&&&Sparse&&0.990&0.924&0.756&0.647&\textbf{0.630}&&0.647&0.647\tabularnewline
~~&&80&Dense&&0.998&0.985&0.946&0.916&\textbf{0.905}&&0.916&0.916\tabularnewline
~~&&&Moderate&&0.998&0.980&0.921&0.867&\textbf{0.708}&&0.867&0.867\tabularnewline
~~&&&Sparse&&0.997&0.977&0.907&0.839&\textbf{0.589}&&0.839&0.839\tabularnewline
\midrule
{\scshape }&&&&&&&&&&&&\tabularnewline
~~&S&240&Dense&&0.999&\textbf{0.998}&1.006&1.034&1.060&&1.034&1.034\tabularnewline
~~&&&Moderate&&0.992&0.945&0.854&\textbf{0.822}&0.836&&0.822&0.822\tabularnewline
~~&&&Sparse&&0.987&0.919&0.771&\textbf{0.694}&0.713&&0.694&0.694\tabularnewline
~~&&80&Dense&&0.999&0.994&0.981&\textbf{0.976}&0.988&&0.976&0.976\tabularnewline
~~&&&Moderate&&0.997&0.975&0.919&0.878&\textbf{0.804}&&0.878&0.878\tabularnewline
~~&&&Sparse&&0.996&0.971&0.903&0.847&\textbf{0.682}&&0.847&0.847\tabularnewline
\bottomrule
\end{tabular}
\caption{MAE ratios of coefficients and covariances to non-sparse BVAR estimates.\label{tab:MAD-A}} 
\begin{minipage}{\textwidth}
 \footnotesize\textbf{Notes:} Bold numbers indicate the smallest MAE ratio. We simulate a DGP for a \textit{small-scale} ($m = 3$), \textit{medium-scale} ($m = 10$) and \textit{large-scale} ($m = 30$) VAR for two different number of observations $T$ and for three different degrees of sparsity (zero parameters as percentage of total number of coefficients $k = m(mp + 1)$ and covariances $w = m(m + 1)/2$, ranging from a dense DGP to a fully sparse DGP. Coefficients of the diagonal of the first lag a non-sparse, as well as the diagonal elements in the variance covariance matrix. 
\end{minipage}\end{center}}
\end{table}


==> MAD_A_lags_05.tex <==
%latex.default(MAD.A.1, file = paste0("MAD_A_lags_", gsub(scale.v.mat.grid,     pattern = "\\.", replacement = ""), ".tex"), title = "",     ctable = FALSE, rgroupTexCmd = "scshape", n.cgroup = n.cgroup,     cgroup = cgroup, colheads = colheads, rgroup = rgroup, n.rgroup = n.rgroup,     caption = "", label = "tab:MAD-AS", size = "tiny", booktabs = TRUE,     numeric.dollar = TRUE, rowname = "", caption.loc = "bottom")%
\begin{table}[!tbp]
{\tiny
\begin{center}
\begin{tabular}{llllclllll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{3}{c}{\bfseries DGP}&\multicolumn{1}{c}{\bfseries }&\multicolumn{5}{c}{\bfseries Sparsify each draw with $\lambda = 1 $}\tabularnewline
\cline{2-4} \cline{6-10}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{M}&\multicolumn{1}{c}{T}&\multicolumn{1}{c}{Sparsity}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{$1^{st}$ lag}&\multicolumn{1}{c}{$2^{nd}$ lag}&\multicolumn{1}{c}{$3^{rd}$ lag}&\multicolumn{1}{c}{$4^{th}$ lag}&\multicolumn{1}{c}{$5^{th}$ lag}\tabularnewline
\midrule
{\scshape }&&&&&&&&&\tabularnewline
~~&L&240&Dense&&1.25&0.94&0.86&0.82&0.79\tabularnewline
~~&&&Moderate&&0.90&0.66&0.59&0.56&0.53\tabularnewline
~~&&&Sparse&&0.51&0.32&0.29&0.27&0.26\tabularnewline
~~&&80&Dense&&1.10&0.94&0.90&0.88&0.86\tabularnewline
~~&&&Moderate&&0.85&0.71&0.67&0.64&0.62\tabularnewline
~~&&&Sparse&&0.54&0.37&0.35&0.33&0.32\tabularnewline
\midrule
{\scshape }&&&&&&&&&\tabularnewline
~~&M&240&Dense&&1.17&0.94&0.78&0.70&0.63\tabularnewline
~~&&&Moderate&&0.86&0.62&0.49&0.42&0.39\tabularnewline
~~&&&Sparse&&0.52&0.28&0.22&0.18&0.17\tabularnewline
~~&&80&Dense&&1.17&0.90&0.80&0.74&0.69\tabularnewline
~~&&&Moderate&&0.85&0.59&0.51&0.47&0.45\tabularnewline
~~&&&Sparse&&0.52&0.26&0.23&0.21&0.20\tabularnewline
\midrule
{\scshape }&&&&&&&&&\tabularnewline
~~&S&240&Dense&&1.12&0.98&0.71&0.57&0.50\tabularnewline
~~&&&Moderate&&0.83&0.61&0.44&0.36&0.32\tabularnewline
~~&&&Sparse&&0.64&0.24&0.16&0.13&0.12\tabularnewline
~~&&80&Dense&&1.08&0.82&0.65&0.56&0.50\tabularnewline
~~&&&Moderate&&0.85&0.51&0.40&0.34&0.32\tabularnewline
~~&&&Sparse&&0.64&0.20&0.14&0.11&0.11\tabularnewline
\bottomrule
\end{tabular}
\caption{MAE ratios of coefficients for each lag to non-sparse BVAR estimates.\label{tab:MAD-A-lag}} 
\end{center}}
\end{table}


==> MAD_A_lags_05_new.tex <==
%latex.default(MAD.A.1, file = paste0("MAD_A_lags_", gsub(scale.v.mat.grid,     pattern = "\\.", replacement = ""), ".tex"), title = "",     ctable = FALSE, rgroupTexCmd = "scshape", n.cgroup = n.cgroup,     cgroup = cgroup, colheads = colheads, rgroup = rgroup, n.rgroup = n.rgroup,     caption = "", label = "tab:MAD-AS", size = "tiny", booktabs = TRUE,     numeric.dollar = TRUE, rowname = "", caption.loc = "bottom")%
\begin{table}[!tbp]
{\tiny
\begin{center}
\begin{tabular}{llllclllll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{3}{c}{\bfseries DGP}&\multicolumn{1}{c}{\bfseries }&\multicolumn{5}{c}{\bfseries Sparsify each draw with $\lambda = 1 $}\tabularnewline
\cline{2-4} \cline{6-10}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{m}&\multicolumn{1}{c}{T}&\multicolumn{1}{c}{Sparsity}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{$1^{st}$ lag}&\multicolumn{1}{c}{$2^{nd}$ lag}&\multicolumn{1}{c}{$3^{rd}$ lag}&\multicolumn{1}{c}{$4^{th}$ lag}&\multicolumn{1}{c}{$5^{th}$ lag}\tabularnewline
\midrule
{\scshape }&&&&&&&&&\tabularnewline
~~&S&80&Sparse&&0.64&0.20&0.14&0.11&0.11\tabularnewline
~~&&&Moderate&&0.85&0.51&0.40&0.34&0.32\tabularnewline
~~&&&Dense&&1.08&0.82&0.65&0.56&0.50\tabularnewline
~~&&240&Sparse&&0.64&0.24&0.16&0.13&0.12\tabularnewline
~~&&&Moderate&&0.83&0.61&0.44&0.36&0.32\tabularnewline
~~&&&Dense&&1.12&0.98&0.71&0.57&0.50\tabularnewline
\midrule
{\scshape }&&&&&&&&&\tabularnewline
~~&M&80&Sparse&&0.52&0.26&0.23&0.21&0.20\tabularnewline
~~&&&Moderate&&0.85&0.59&0.51&0.47&0.45\tabularnewline
~~&&&Dense&&1.17&0.90&0.80&0.74&0.69\tabularnewline
~~&&240&Sparse&&0.52&0.28&0.22&0.18&0.17\tabularnewline
~~&&&Moderate&&0.86&0.62&0.49&0.42&0.39\tabularnewline
~~&&&Dense&&1.17&0.94&0.78&0.70&0.63\tabularnewline
\midrule
{\scshape }&&&&&&&&&\tabularnewline
~~&L&80&Sparse&&0.54&0.37&0.35&0.33&0.32\tabularnewline
~~&&&Moderate&&0.85&0.71&0.67&0.64&0.62\tabularnewline
~~&&&Dense&&1.10&0.94&0.90&0.88&0.86\tabularnewline
~~&&240&Sparse&&0.51&0.32&0.29&0.27&0.26\tabularnewline
~~&&&Moderate&&0.90&0.66&0.59&0.56&0.53\tabularnewline
~~&&&Dense&&1.25&0.94&0.86&0.82&0.79\tabularnewline
\bottomrule
\end{tabular}
\caption{MAE ratios of coefficients for each lag to non-sparse BVAR estimates.\label{tab:MAD-A-lag}} 
\end{center}}
\end{table}


==> MAD_A_lags_4.tex <==
%latex.default(MAD.A.1, file = paste0("MAD_A_lags_", gsub(scale.v.mat.grid,     pattern = "\\.", replacement = ""), ".tex"), title = "",     ctable = FALSE, rgroupTexCmd = "scshape", n.cgroup = n.cgroup,     cgroup = cgroup, colheads = colheads, rgroup = rgroup, n.rgroup = n.rgroup,     caption = "", label = "tab:MAD-AS", size = "tiny", booktabs = TRUE,     numeric.dollar = TRUE, rowname = "", caption.loc = "bottom")%
\begin{table}[!tbp]
{\tiny
\begin{center}
\begin{tabular}{llllclllll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{3}{c}{\bfseries DGP}&\multicolumn{1}{c}{\bfseries }&\multicolumn{5}{c}{\bfseries Sparsify each draw with $\lambda = 1 $}\tabularnewline
\cline{2-4} \cline{6-10}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{M}&\multicolumn{1}{c}{T}&\multicolumn{1}{c}{Sparsity}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{$1^{st}$ lag}&\multicolumn{1}{c}{$2^{nd}$ lag}&\multicolumn{1}{c}{$3^{rd}$ lag}&\multicolumn{1}{c}{$4^{th}$ lag}&\multicolumn{1}{c}{$5^{th}$ lag}\tabularnewline
\midrule
{\scshape }&&&&&&&&&\tabularnewline
~~&L&240&Dense&&1.15&0.94&0.86&0.82&0.79\tabularnewline
~~&&&Moderate&&0.84&0.65&0.59&0.55&0.53\tabularnewline
~~&&&Sparse&&0.50&0.32&0.29&0.27&0.26\tabularnewline
~~&&80&Dense&&1.10&0.94&0.90&0.88&0.86\tabularnewline
~~&&&Moderate&&0.85&0.71&0.67&0.64&0.62\tabularnewline
~~&&&Sparse&&0.54&0.37&0.35&0.33&0.32\tabularnewline
\midrule
{\scshape }&&&&&&&&&\tabularnewline
~~&M&240&Dense&&1.03&0.94&0.77&0.68&0.62\tabularnewline
~~&&&Moderate&&0.79&0.62&0.49&0.42&0.38\tabularnewline
~~&&&Sparse&&0.57&0.28&0.22&0.18&0.17\tabularnewline
~~&&80&Dense&&1.04&0.90&0.79&0.73&0.69\tabularnewline
~~&&&Moderate&&0.81&0.58&0.51&0.47&0.44\tabularnewline
~~&&&Sparse&&0.60&0.26&0.23&0.21&0.20\tabularnewline
\midrule
{\scshape }&&&&&&&&&\tabularnewline
~~&S&240&Dense&&1.00&0.97&0.72&0.58&0.50\tabularnewline
~~&&&Moderate&&0.82&0.59&0.45&0.36&0.32\tabularnewline
~~&&&Sparse&&0.70&0.29&0.16&0.13&0.12\tabularnewline
~~&&80&Dense&&1.00&0.84&0.65&0.56&0.49\tabularnewline
~~&&&Moderate&&0.85&0.53&0.39&0.34&0.32\tabularnewline
~~&&&Sparse&&0.74&0.26&0.14&0.11&0.11\tabularnewline
\bottomrule
\end{tabular}
\caption{MAE ratios of coefficients for each lag to non-sparse BVAR estimates.\label{tab:MAD-A-lag}} 
\end{center}}
\end{table}


==> MAD_sd_05.tex <==
%latex.default(MAD.sd, file = paste0("MAD_sd_", gsub(scale.v.mat.grid,     pattern = "\\.", replacement = ""), ".tex"), title = "",     ctable = FALSE, rgroupTexCmd = "scshape", n.cgroup = n.cgroup,     cgroup = cgroup, colheads = colheads, rgroup = rgroup, n.rgroup = n.rgroup,     caption = "", label = "tab:MAD-AS", size = "tiny", booktabs = TRUE,     numeric.dollar = TRUE, rowname = "", caption.loc = "bottom")%
\begin{table}[!tbp]
{\tiny
\begin{center}
\begin{tabular}{lllllcllll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{4}{c}{\bfseries DGP}&\multicolumn{1}{c}{\bfseries }&\multicolumn{4}{c}{\bfseries Standard deviation of MAEs}\tabularnewline
\cline{2-5} \cline{7-10}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{M}&\multicolumn{1}{c}{T}&\multicolumn{1}{c}{Sigma}&\multicolumn{1}{c}{Sparsity}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{A - MIN}&\multicolumn{1}{c}{A - MIN-SAVS}&\multicolumn{1}{c}{$\Sigma$ - MIN}&\multicolumn{1}{c}{$\Sigma$ - MIN-SAVS}\tabularnewline
\midrule
{\scshape }&&&&&&&&&\tabularnewline
~~&L&240&0.5&Dense&&0.0003&0.0025&0.0009&0.0009\tabularnewline
~~&&&&Moderate&&0.0003&0.0003&0.0007&0.0007\tabularnewline
~~&&&&Sparse&&0.0002&0.0002&0.0006&0.0006\tabularnewline
~~&&80&&Dense&&0.0004&0.0004&0.0015&0.0014\tabularnewline
~~&&&&Moderate&&0.0003&0.0004&0.0013&0.0013\tabularnewline
~~&&&&Sparse&&0.0002&0.0002&0.0009&0.0010\tabularnewline
\midrule
{\scshape }&&&&&&&&&\tabularnewline
~~&M&240&&Dense&&0.0017&0.0374&0.0029&0.0029\tabularnewline
~~&&&&Moderate&&0.0015&0.0011&0.0022&0.0021\tabularnewline
~~&&&&Sparse&&0.0012&0.0007&0.0020&0.0018\tabularnewline
~~&&80&&Dense&&0.0023&0.0027&0.0052&0.0053\tabularnewline
~~&&&&Moderate&&0.0018&0.0015&0.0043&0.0042\tabularnewline
~~&&&&Sparse&&0.0015&0.0012&0.0033&0.0035\tabularnewline
\midrule
{\scshape }&&&&&&&&&\tabularnewline
~~&S&240&&Dense&&0.0068&0.0045&0.0071&0.0074\tabularnewline
~~&&&&Moderate&&0.0060&0.0036&0.0073&0.0069\tabularnewline
~~&&&&Sparse&&0.0048&0.0025&0.0073&0.0061\tabularnewline
~~&&80&&Dense&&0.0094&0.0070&0.0134&0.0135\tabularnewline
~~&&&&Moderate&&0.0082&0.0059&0.0122&0.0121\tabularnewline
~~&&&&Sparse&&0.0076&0.0050&0.0119&0.0117\tabularnewline
\bottomrule
\end{tabular}
\caption{\label{tab:MAD-AS}}\end{center}}
\end{table}


==> MAD_sd_4.tex <==
%latex.default(MAD.sd, file = paste0("MAD_sd_", gsub(scale.v.mat.grid,     pattern = "\\.", replacement = ""), ".tex"), title = "",     ctable = FALSE, rgroupTexCmd = "scshape", n.cgroup = n.cgroup,     cgroup = cgroup, colheads = colheads, rgroup = rgroup, n.rgroup = n.rgroup,     caption = "", label = "tab:MAD-AS", size = "tiny", booktabs = TRUE,     numeric.dollar = TRUE, rowname = "", caption.loc = "bottom")%
\begin{table}[!tbp]
{\tiny
\begin{center}
\begin{tabular}{lllllcllll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{4}{c}{\bfseries DGP}&\multicolumn{1}{c}{\bfseries }&\multicolumn{4}{c}{\bfseries Standard deviation of MAEs}\tabularnewline
\cline{2-5} \cline{7-10}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{M}&\multicolumn{1}{c}{T}&\multicolumn{1}{c}{Sigma}&\multicolumn{1}{c}{Sparsity}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{A - MIN}&\multicolumn{1}{c}{A - MIN-SAVS}&\multicolumn{1}{c}{$\Sigma$ - MIN}&\multicolumn{1}{c}{$\Sigma$ - MIN-SAVS}\tabularnewline
\midrule
{\scshape }&&&&&&&&&\tabularnewline
~~&L&240&4&Dense&&0.0003&0.0026&0.0019&0.0015\tabularnewline
~~&&&&Moderate&&0.0003&0.0003&0.0017&0.0015\tabularnewline
~~&&&&Sparse&&0.0002&0.0002&0.0018&0.0016\tabularnewline
~~&&80&&Dense&&0.0005&0.0010&0.0034&0.0033\tabularnewline
~~&&&&Moderate&&0.0004&0.0004&0.0032&0.0033\tabularnewline
~~&&&&Sparse&&0.0003&0.0003&0.0027&0.0028\tabularnewline
\midrule
{\scshape }&&&&&&&&&\tabularnewline
~~&M&240&&Dense&&0.0015&0.0574&0.0061&0.0053\tabularnewline
~~&&&&Moderate&&0.0015&0.0011&0.0053&0.0049\tabularnewline
~~&&&&Sparse&&0.0013&0.0010&0.0053&0.0047\tabularnewline
~~&&80&&Dense&&0.0024&0.0323&0.0108&0.0102\tabularnewline
~~&&&&Moderate&&0.0020&0.0019&0.0104&0.0103\tabularnewline
~~&&&&Sparse&&0.0019&0.0018&0.0091&0.0096\tabularnewline
\midrule
{\scshape }&&&&&&&&&\tabularnewline
~~&S&240&&Dense&&0.0062&0.0050&0.0177&0.0161\tabularnewline
~~&&&&Moderate&&0.0059&0.0041&0.0198&0.0177\tabularnewline
~~&&&&Sparse&&0.0056&0.0044&0.0205&0.0172\tabularnewline
~~&&80&&Dense&&0.0095&0.0089&0.0326&0.0309\tabularnewline
~~&&&&Moderate&&0.0096&0.0087&0.0331&0.0325\tabularnewline
~~&&&&Sparse&&0.0097&0.0088&0.0337&0.0331\tabularnewline
\bottomrule
\end{tabular}
\caption{\label{tab:MAD-AS}}\end{center}}
\end{table}


==> RMSE_final.tex <==
%latex.default(rmse.all, file = paste0("RMSE", "_", eval.type,     ".tex"), title = "", ctable = FALSE, rgroupTexCmd = "scshape",     n.cgroup = n.cgroup, cgroup = cgroup, colheads = colheads,     rgroup = rgroup, n.rgroup = n.rgroup, caption = "", label = "tab:point",     size = "tiny", rownamesTexCmd = my.rownamesTexCmd, rowname = "",     booktabs = TRUE, numeric.dollar = TRUE, caption.loc = "bottom",     landscape = TRUE)%
\begin{landscape}\begin{table}[!tbp]
{\tiny
\begin{center}
\scalebox{0.95}{
\begin{tabular}{llclllclllclllclll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{1}{c}{\bfseries Spec.}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Avg.}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal 1-step-ahead}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal 4-step-ahead}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal 8-step-ahead}\tabularnewline
\cline{2-2} \cline{4-6} \cline{8-10} \cline{12-14} \cline{16-18}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{1-step ahead}&\multicolumn{1}{c}{4-step ahead}&\multicolumn{1}{c}{8-step ahead}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{ CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{ CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}\tabularnewline
\midrule
{\scshape Small}&&&&&&&&&&&&&&&&&\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   0.980&   1.003&   1.000&   &   1.008&   \textbf{0.975}&   0.951&   &   1.008&   0.996&   1.049&   &   1.010&   0.994&   1.024\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   0.977&   0.999&   0.994&   &   1.002&   0.992&   0.833&   &   1.021&   0.995&   0.973&   &   0.979&   0.994***&   1.039\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   \textbf{0.976}&   1.000&   0.997&   &   1.005&   1.000&   0.756**&   &   1.002&   1.000&   0.995&   &   1.015&   0.984&   1.077\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   0.981&   0.996&   0.982&   &   1.004&   1.011&   0.736***&   &   0.996&   0.998&   0.983&   &   0.984&   0.977&   1.033\tabularnewline
\shadeRow   ~~&   SSVS&   &   0.991&   1.030&   0.987&   &   1.018&   0.989&   0.948&   &   1.059&   1.021&   1.029&   &   1.017&   0.975&   1.017\tabularnewline
\midrule
{\scshape FAVAR}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.041&   1.031**&   1.006&   &   0.937&   1.022*&   1.317&   &   1.083***&   1.020&   0.977&   &   1.083&   0.987&   \textbf{0.943}\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   1.024&   1.013&   1.008&   &   0.905&   1.015&   1.272&   &   1.043&   1.010&   0.959&   &   1.020&   1.000&   1.053\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   1.025&   1.019&   0.990&   &   0.903&   1.037&   1.185&   &   1.081**&   0.996&   1.042&   &   0.999&   0.983&   1.034\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.047&   1.027&   1.001&   &   0.909&   1.066*&   1.201&   &   1.110**&   0.993*&   1.095&   &   1.001&   0.995&   1.066\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   1.064&   1.014&   0.995&   &   0.903&   1.092*&   1.203&   &   1.055&   1.000&   1.017&   &   0.980&   0.992**&   1.072\tabularnewline
\shadeRow   ~~&   SSVS&   &   1.164***&   1.181***&   1.154***&   &   0.857&   1.213***&   1.411***&   &   1.116***&   1.198***&   1.204**&   &   1.074*&   1.161***&   1.317***\tabularnewline
\midrule
{\scshape Medium}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.067&   0.985&   1.006&   &   0.844&   1.112**&   1.216&   &   1.011&   0.980&   0.960*&   &   1.039&   0.996&   1.010\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   1.041&   0.983&   0.997&   &   \textbf{0.815**}&   1.114**&   1.040&   &   0.996&   0.982&   0.953&   &   1.007&   0.993&   1.011\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   1.011&   1.008&   0.985&   &   0.837***&   1.098**&   0.817***&   &   1.020&   1.004&   1.012&   &   1.010&   0.972&   1.051\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.002&   0.999&   \textbf{0.972}&   &   0.939&   1.065&   \textbf{0.725***}&   &   1.011&   0.995&   0.994&   &   0.978&   \textbf{0.964}&   1.027\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   1.025&   0.993&   0.988&   &   1.013&   1.070&   0.759**&   &   1.004&   0.992&   0.975&   &   0.995&   0.981&   1.037\tabularnewline
\shadeRow   ~~&   SSVS&   &   1.189***&   1.223***&   1.215***&   &   0.938&   1.240***&   1.353***&   &   1.147*&   1.216***&   1.472***&   &   1.129&   1.212***&   1.490***\tabularnewline
\midrule
{\scshape Large ($\theta_1 = 0.025$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.000&   \textbf{0.978}&   0.995&   &   0.854**&   1.068&   0.876&   &   0.994&   \textbf{0.975}&   0.956&   &   1.029&   0.983&   1.010\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   1.041&   0.994&   0.983&   &   0.996&   1.096*&   0.782**&   &   1.020&   0.989&   0.963&   &   0.990&   0.978&   1.023\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   1.055&   1.003&   0.991&   &   1.005&   1.105*&   0.848**&   &   1.020&   1.002&   0.966&   &   0.988&   0.986&   1.061\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.045&   0.990&   0.983&   &   1.021&   1.087&   0.833*&   &   0.992&   0.992&   0.967&   &   0.969&   0.982&   1.035\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   1.046&   0.999&   0.980&   &   1.025&   1.085*&   0.851*&   &   1.010&   1.001&   0.947&   &   \textbf{0.966*}&   0.980&   1.026\tabularnewline
\midrule
{\scshape Large ($\theta_1 = 0.050$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.023&   1.000&   0.984&   &   0.881&   1.055&   1.110&   &   1.010&   1.000&   0.970&   &   1.011&   0.976&   0.974\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   1.020&   0.994&   0.983&   &   0.891*&   1.091&   0.848**&   &   0.995&   0.995&   0.975&   &   1.007&   0.972&   1.023\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   1.039&   0.995&   0.984&   &   0.986&   1.092*&   0.823**&   &   1.023&   0.987&   0.992&   &   0.982&   0.982&   1.011\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.052&   1.003&   0.983*&   &   1.032&   1.091&   0.854*&   &   1.006&   1.003&   0.987&   &   0.981*&   0.981&   1.013\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   1.043&   0.993&   0.986&   &   1.020&   1.084*&   0.837*&   &   0.998&   0.993&   0.978&   &   0.990&   0.980&   1.035\tabularnewline
\midrule
{\scshape Large ($\theta_1 = 0.075$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.037&   0.997&   1.011**&   &   0.921&   1.042&   1.222&   &   1.004&   0.997&   0.983&   &   1.059*&   0.995&   1.023\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   1.039&   0.984&   0.984&   &   0.885&   1.104*&   0.963&   &   \textbf{0.982}&   0.988&   0.961&   &   0.973*&   0.983&   1.036\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   1.029&   0.993&   0.985&   &   0.981&   1.084*&   0.780**&   &   1.003&   0.996&   \textbf{0.943}&   &   0.984&   0.979&   1.042\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.050&   0.994&   0.984&   &   1.056&   1.087&   0.799**&   &   1.004&   0.996&   0.949*&   &   0.993&   0.980&   0.996\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   1.050&   0.993&   0.990&   &   1.036&   1.094*&   0.806**&   &   1.016&   0.989&   0.957&   &   0.990&   0.988&   1.016\tabularnewline
\bottomrule
\end{tabular}}
\caption{RMSE ratios relative to the \textit{small-scale} BVAR with a Minnesota prior. \label{tab:RMSE}}
\begin{minipage}{\linewidth}
\footnotesize \textbf{Notes}: Bold numbers indicate lowest RMSE ratios for each horizon and target variable (and therefore best performing models over the full hold-out sample). Gray shaded rows denote non-sparsified models. Asterisks indicate statistical significance for each model relative to the benchmark at the $1$ ($^{***}$), $5$ ($^{**}$) and $10$ ($^{*}$) percent significance levels. 
\end{minipage}\end{center}}
\end{table}\end{landscape}


==> RMSE_full.tex <==
%latex.default(rmse.all, file = paste0("RMSE", "_", eval.type,     ".tex"), title = "", ctable = FALSE, rgroupTexCmd = "scshape",     n.cgroup = n.cgroup, cgroup = cgroup, colheads = colheads,     rgroup = rgroup, n.rgroup = n.rgroup, caption = "", label = "tab:point",     size = "tiny", rownamesTexCmd = my.rownamesTexCmd, rowname = "",     booktabs = TRUE, numeric.dollar = TRUE, caption.loc = "bottom",     landscape = TRUE)%
\begin{landscape}\begin{table}[!tbp]
{\tiny
\begin{center}
\scalebox{0.9}{
\begin{tabular}{llclllclllclllclll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{1}{c}{\bfseries Spec.}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Avg.}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal 1-step-ahead}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal 4-step-ahead}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries Marginal 8-step-ahead}\tabularnewline
\cline{2-2} \cline{4-6} \cline{8-10} \cline{12-14} \cline{16-18}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{1-step ahead}&\multicolumn{1}{c}{4-step ahead}&\multicolumn{1}{c}{8-step ahead}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{ CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{ CPIAUCSL}&\multicolumn{1}{c}{FEDFUNDS}\tabularnewline
\midrule
{\scshape Small}&&&&&&&&&&&&&&&&&\tabularnewline
   ~~&   MIN - $\lambda = 0.005$&   &   0.999&   1.006&   0.995&   &   1.016&   0.987&   1.029&   &   1.034&   0.999&   0.997&   &   0.983&   0.998&   1.010\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   0.980&   1.003&   1.000&   &   1.008&   0.975&   0.951&   &   1.008&   0.996&   1.049&   &   1.010&   0.994&   1.024\tabularnewline
   ~~&   MIN - $\lambda = 0.05$&   &   \textbf{0.974}&   1.008&   0.995&   &   1.022&   \textbf{0.966}&   0.912&   &   1.025&   1.001&   1.029&   &   0.994&   0.989&   1.055\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   0.977&   0.999&   0.994&   &   1.002&   0.992&   0.833&   &   1.021&   0.995&   0.973&   &   0.979&   0.994***&   1.039\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   0.976&   1.000&   0.997&   &   1.005&   1.000&   0.756**&   &   1.002&   1.000&   0.995&   &   1.015&   0.984&   1.077\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   0.981&   0.996&   0.982&   &   1.004&   1.011&   0.736***&   &   0.996&   0.998&   0.983&   &   0.984&   0.977&   1.033\tabularnewline
\shadeRow   ~~&   SSVS&   &   0.991&   1.030&   0.987&   &   1.018&   0.989&   0.948&   &   1.059&   1.021&   1.029&   &   1.017&   0.975&   1.017\tabularnewline
\midrule
{\scshape FAVAR}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.041&   1.031**&   1.006&   &   0.937&   1.022*&   1.317&   &   1.083***&   1.020&   0.977&   &   1.083&   0.987&   \textbf{0.943}\tabularnewline
   ~~&   MIN - $\lambda = 0.005$&   &   1.022&   1.019&   0.994&   &   0.904&   1.014&   1.269&   &   1.091***&   1.000&   0.982&   &   1.028&   0.976&   1.073\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   1.024&   1.013&   1.008&   &   0.905&   1.015&   1.272&   &   1.043&   1.010&   0.959&   &   1.020&   1.000&   1.053\tabularnewline
   ~~&   MIN - $\lambda = 0.05$&   &   1.021&   1.017&   0.994&   &   0.911&   1.013&   1.252&   &   1.095**&   0.990&   1.039&   &   1.023&   0.980&   1.038\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   1.025&   1.019&   0.990&   &   0.903&   1.037&   1.185&   &   1.081**&   0.996&   1.042&   &   0.999&   0.983&   1.034\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.047&   1.027&   1.001&   &   0.909&   1.066*&   1.201&   &   1.110**&   0.993*&   1.095&   &   1.001&   0.995&   1.066\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   1.064&   1.014&   0.995&   &   0.903&   1.092*&   1.203&   &   1.055&   1.000&   1.017&   &   0.980&   0.992**&   1.072\tabularnewline
\shadeRow   ~~&   SSVS&   &   1.164***&   1.181***&   1.154***&   &   0.857&   1.213***&   1.411***&   &   1.116***&   1.198***&   1.204**&   &   1.074*&   1.161***&   1.317***\tabularnewline
\midrule
{\scshape Medium}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.067&   0.985&   1.006&   &   0.844&   1.112**&   1.216&   &   1.011&   0.980&   0.960*&   &   1.039&   0.996&   1.010\tabularnewline
   ~~&   MIN - $\lambda = 0.005$&   &   1.039&   1.001&   0.994&   &   \textbf{0.796***}&   1.104**&   1.105&   &   1.008&   0.997&   1.016&   &   0.997&   0.986&   1.070\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   1.041&   0.983&   0.997&   &   0.815**&   1.114**&   1.040&   &   0.996&   0.982&   0.953&   &   1.007&   0.993&   1.011\tabularnewline
   ~~&   MIN - $\lambda = 0.05$&   &   0.991&   0.997&   0.987&   &   0.804***&   1.073**&   0.854***&   &   1.007&   1.000&   0.943&   &   0.985&   0.984&   1.033\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   1.011&   1.008&   0.985&   &   0.837***&   1.098**&   0.817***&   &   1.020&   1.004&   1.012&   &   1.010&   0.972&   1.051\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.002&   0.999&   \textbf{0.972}&   &   0.939&   1.065&   \textbf{0.725***}&   &   1.011&   0.995&   0.994&   &   0.978&   \textbf{0.964}&   1.027\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   1.025&   0.993&   0.988&   &   1.013&   1.070&   0.759**&   &   1.004&   0.992&   0.975&   &   0.995&   0.981&   1.037\tabularnewline
\shadeRow   ~~&   SSVS&   &   1.189***&   1.223***&   1.215***&   &   0.938&   1.240***&   1.353***&   &   1.147*&   1.216***&   1.472***&   &   1.129&   1.212***&   1.490***\tabularnewline
\midrule
{\scshape Xlarge ($\theta_1 = 0.025$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.000&   \textbf{0.978}&   0.995&   &   0.854**&   1.068&   0.876&   &   0.994&   \textbf{0.975}&   0.956&   &   1.029&   0.983&   1.010\tabularnewline
   ~~&   MIN - $\lambda = 0.005$&   &   1.022&   0.991&   0.983&   &   0.946**&   1.088*&   0.766***&   &   0.990&   0.992&   0.976&   &   1.004&   0.975&   0.994\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   1.041&   0.994&   0.983&   &   0.996&   1.096*&   0.782**&   &   1.020&   0.989&   0.963&   &   0.990&   0.978&   1.023\tabularnewline
   ~~&   MIN - $\lambda = 0.05$&   &   1.046&   0.993&   0.994&   &   1.037&   1.086&   0.806**&   &   0.988&   0.999&   0.949&   &   1.010&   0.985&   1.039\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   1.055&   1.003&   0.991&   &   1.005&   1.105*&   0.848**&   &   1.020&   1.002&   0.966&   &   0.988&   0.986&   1.061\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.045&   0.990&   0.983&   &   1.021&   1.087&   0.833*&   &   0.992&   0.992&   0.967&   &   0.969&   0.982&   1.035\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   1.046&   0.999&   0.980&   &   1.025&   1.085*&   0.851*&   &   1.010&   1.001&   0.947&   &   \textbf{0.966*}&   0.980&   1.026\tabularnewline
\midrule
{\scshape Xlarge ($\theta_1 = 0.050$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.023&   1.000&   0.984&   &   0.881&   1.055&   1.110&   &   1.010&   1.000&   0.970&   &   1.011&   0.976&   0.974\tabularnewline
   ~~&   MIN - $\lambda = 0.005$&   &   1.010&   0.991&   0.983&   &   0.889&   1.072&   0.877**&   &   1.011&   0.992&   \textbf{0.923*}&   &   0.975&   0.980&   1.043\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   1.020&   0.994&   0.983&   &   0.891*&   1.091&   0.848**&   &   0.995&   0.995&   0.975&   &   1.007&   0.972&   1.023\tabularnewline
   ~~&   MIN - $\lambda = 0.05$&   &   1.037&   0.989&   0.997&   &   0.977&   1.097*&   0.778***&   &   0.998&   0.989&   0.960&   &   0.991&   0.994&   1.053\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   1.039&   0.995&   0.984&   &   0.986&   1.092*&   0.823**&   &   1.023&   0.987&   0.992&   &   0.982&   0.982&   1.011\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.052&   1.003&   0.983*&   &   1.032&   1.091&   0.854*&   &   1.006&   1.003&   0.987&   &   0.981*&   0.981&   1.013\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   1.043&   0.993&   0.986&   &   1.020&   1.084*&   0.837*&   &   0.998&   0.993&   0.978&   &   0.990&   0.980&   1.035\tabularnewline
\midrule
{\scshape Xlarge ($\theta_1 = 0.075$)}&&&&&&&&&&&&&&&&&\tabularnewline
\shadeRow   ~~&   MIN&   &   1.037&   0.997&   1.011**&   &   0.921&   1.042&   1.222&   &   1.004&   0.997&   0.983&   &   1.059*&   0.995&   1.023\tabularnewline
   ~~&   MIN - $\lambda = 0.005$&   &   1.041&   1.002&   0.973&   &   0.881&   1.095*&   1.039&   &   0.984&   1.013&   0.952&   &   0.978&   0.967&   1.029\tabularnewline
   ~~&   MIN - $\lambda = 0.01$&   &   1.039&   0.984&   0.984&   &   0.885&   1.104*&   0.963&   &   \textbf{0.982}&   0.988&   0.961&   &   0.973*&   0.983&   1.036\tabularnewline
   ~~&   MIN - $\lambda = 0.05$&   &   1.019&   0.992&   0.993&   &   0.943&   1.079&   0.802**&   &   1.014&   0.987&   0.977&   &   0.998&   0.985&   1.062\tabularnewline
   ~~&   MIN - $\lambda = 0.1$&   &   1.029&   0.993&   0.985&   &   0.981&   1.084*&   0.780**&   &   1.003&   0.996&   0.943&   &   0.984&   0.979&   1.042\tabularnewline
   ~~&   MIN - $\lambda = 0.5$&   &   1.050&   0.994&   0.984&   &   1.056&   1.087&   0.799**&   &   1.004&   0.996&   0.949*&   &   0.993&   0.980&   0.996\tabularnewline
   ~~&   MIN - $\lambda = 1$&   &   1.050&   0.993&   0.990&   &   1.036&   1.094*&   0.806**&   &   1.016&   0.989&   0.957&   &   0.990&   0.988&   1.016\tabularnewline
\bottomrule
\end{tabular}}
\caption{RMSE ratios relative to the \textit{small-scale} BVAR with a Minnesota prior. \label{tab:RMSE}}
\begin{minipage}{\linewidth}
\footnotesize \textbf{Notes}: Bold numbers indicate lowest RMSE ratios for each horizon and target variable (and therefore best performing models over the full hold-out sample). Gray shaded rows denote non-sparsified models. Asterisks indicate statistical significance for each model relative to the benchmark at the $1$ ($^{***}$), $5$ ($^{**}$) and $10$ ($^{*}$) percent significance levels. 
\end{minipage}\end{center}}
\end{table}\end{landscape}


==> best_LPS.tex <==
\begin{table}[!htb]
{\tiny
\begin{center}
\scalebox{0.9}{
\begin{tabular}{lllllllllllll}
\toprule
\multicolumn{1}{l}{\bfseries Variable}&\multicolumn{1}{c}{}& \multicolumn{2}{c}{\bfseries One-quarter-ahead}&\multicolumn{1}{c}{}&\multicolumn{2}{c}{\bfseries One-year-ahead}&\multicolumn{1}{c}{}&\multicolumn{2}{c}{\bfseries Two-year-ahead} \tabularnewline
\cline{3-4} \cline{6-7} \cline{9-10}
\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{c}{Size}&\multicolumn{1}{c}{Spec.}&\multicolumn{1}{l}{}&\multicolumn{1}{c}{Size}&\multicolumn{1}{c}{Spec.}&\multicolumn{1}{l}{}&\multicolumn{1}{c}{Size}&\multicolumn{1}{c}{Spec.} \tabularnewline
\midrule
\textbf{LPSs} & & & & & & & & & \\[5 pt]
Joint && \texttt{M-VAR}& \texttt{MIN - $\lambda = 0.1$}  && \texttt{M-VAR}& \texttt{MIN - $\lambda = 1$} && \texttt{M-VAR}& \texttt{MIN - $\lambda = 0.5$}  \\[5 pt]
GDPC1 && \texttt{M-VAR}& \texttt{MIN - $\lambda = 0.01$}  && \texttt{L-VAR ($\theta_1 = 0.075$)}& \texttt{MIN - $\lambda = 0.01$} && \texttt{L-VAR ($\theta_1 = 0.075$)}& \texttt{MIN - $\lambda = 0.01$} \\
 CPIAUCSL && \texttt{FA-VAR}& \texttt{MIN - $\lambda = 0.01$}  && \texttt{S-VAR}& \texttt{SSVS}  && \texttt{S-VAR}& \texttt{SSVS}   \\
 FEDFUNDS && \texttt{L-VAR ($\theta_1 = 0.075$)}& \texttt{MIN - $\lambda = 1$} && \texttt{L-VAR ($\theta_1 = 0.075$)}& \texttt{MIN - $\lambda = 1$}  &&\texttt{L-VAR ($\theta_1 = 0.075$)}& \texttt{MIN - $\lambda = 1$} \\
\bottomrule
\end{tabular}}
\caption{Overview of the best performing models for density forecasts, indicated by bold numbers in \autoref{tab:LPS}. \label{tab:bestdens}}
\end{center}}
\end{table}

==> best_RMSE.tex <==
\begin{table}[!htb]
{\tiny
\begin{center}
\scalebox{0.9}{
\begin{tabular}{lllllllllllll}
\toprule
\multicolumn{1}{l}{\bfseries Variable}&\multicolumn{1}{c}{}& \multicolumn{2}{c}{\bfseries One-quarter-ahead}&\multicolumn{1}{c}{}&\multicolumn{2}{c}{\bfseries One-year-ahead}&\multicolumn{1}{c}{}&\multicolumn{2}{c}{\bfseries Two-year-ahead} \tabularnewline
\cline{3-4} \cline{6-7} \cline{9-10}
\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{c}{Size}&\multicolumn{1}{c}{Spec.}&\multicolumn{1}{l}{}&\multicolumn{1}{c}{Size}&\multicolumn{1}{c}{Spec.}&\multicolumn{1}{l}{}&\multicolumn{1}{c}{Size}&\multicolumn{1}{c}{Spec.} \tabularnewline
\midrule
\textbf{RMSEs} & & & & & & & & & \\[5 pt]
Avg. && \texttt{S-VAR}& \texttt{MIN - $\lambda = 0.5$}  && \texttt{L-VAR ($\theta_1 = 0.025$)}& \texttt{MIN} && \texttt{M-VAR}& \texttt{MIN - $\lambda = 0.5$}  \\[5 pt]
GDPC1 && \texttt{M-VAR}& \texttt{MIN - $\lambda = 0.01$}  && \texttt{L-VAR ($\theta_1 = 0.075$)}& \texttt{MIN - $\lambda = 0.01$} && \texttt{L-VAR ($\theta_1 = 0.025$)}& \texttt{MIN - $\lambda = 1$} \\
 CPIAUCSL && \texttt{S-VAR}& \texttt{MIN - $\lambda = 0.01$}  && \texttt{L-VAR ($\theta_1 = 0.025$)}& \texttt{MIN}  && \texttt{M-VAR}& \texttt{MIN - $\lambda = 0.5$}   \\
 FEDFUNDS && \texttt{M-VAR}& \texttt{MIN - $\lambda = 0.5$} && \texttt{L-VAR ($\theta_1 = 0.075$)}& \texttt{MIN - $\lambda = 0.1$}  &&\texttt{FA-VAR}& \texttt{MIN} \\
\bottomrule
\end{tabular}}
\caption{Overview of the best performing models for point forecasts, indicated by bold numbers in \autoref{tab:RMSE}. \label{tab:bestpoint}}
\end{center}}
\end{table}

==> data_desc1.tex <==
%latex.default(mc.cracken.1, file = "data_desc1.tex", title = "",     ctable = FALSE, rgroupTexCmd = "scshape", rgroup = rgroup,     n.rgroup = n.rgroup.1, caption = "Data description", label = "tab:data-descr1",     size = "tiny", booktabs = TRUE, numeric.dollar = TRUE, rowname = "",     colnames = "", caption.loc = "bottom", landscape = FALSE)%
\begin{table}[h]
{\tiny
\begin{center}
\scalebox{0.8}{
\begin{tabular}{lllrlll}
\toprule
\multicolumn{1}{l}{\ }&\multicolumn{1}{c}{\ FRED.Mnemonic}&\multicolumn{1}{c}{\ Description}&\multicolumn{1}{c}{\ Trans I(0)}&\multicolumn{1}{c}{\ SMALL}&\multicolumn{1}{c}{\ MEDIUM}&\multicolumn{1}{c}{\ LARGE}\tabularnewline
\midrule
{\scshape Slow}&&&&&&\tabularnewline
~~&GDPC1&Real Gross Domestic Product&$5$&x&x&x\tabularnewline
~~&PCECC96&Real Personal Consumption Expenditures&$5$&&x&x\tabularnewline
~~&PCDGx&Real personal consumption expenditures:  Durable goods &$5$&&&x\tabularnewline
~~&PCESVx&Real Personal Consumption Expenditures:  Services &$5$&&&x\tabularnewline
~~&PCNDx&Real Personal Consumption Expenditures:  Nondurable Goods &$5$&&&x\tabularnewline
~~&GPDIC1&Real Gross Private Domestic Investment&$5$&&&x\tabularnewline
~~&FPIx&Real private fixed investment &$5$&&x&x\tabularnewline
~~&Y033RC1Q027SBEAx&Real Gross Private Domestic Investment:  Fixed Investment:  Nonresidential Equipment&$5$&&&x\tabularnewline
~~&PNFIx&Real private fixed investment:  Nonresidential &$5$&&&x\tabularnewline
~~&PRFIx&Real private fixed investment:  Residential &$5$&&&x\tabularnewline
~~&A014RE1Q156NBEA&Shares of gross domestic product:  Gross private domestic investment: Change
in private inventories&$1$&&&x\tabularnewline
~~&GCEC1&Real Government Consumption Expenditures and Gross Investment&$5$&&x&x\tabularnewline
~~&A823RL1Q225SBEA&Real Government Consumption Expenditures and Gross Investment:  Federal&$1$&&&x\tabularnewline
~~&FGRECPTx&Real Federal Government Current Receipts &$5$&&&x\tabularnewline
~~&SLCEx&Real government state and local consumption expenditures &$5$&&&x\tabularnewline
~~&EXPGSC1&Real Exports of Goods and Services&$5$&&&x\tabularnewline
~~&IMPGSC1&Real Imports of Goods and Services&$5$&&&x\tabularnewline
~~&DPIC96&Real Disposable Personal Income&$5$&&&x\tabularnewline
~~&OUTNFB&Nonfarm Business Sector:  Real Output&$5$&&&x\tabularnewline
~~&OUTBS&Business Sector:  Real Output&$5$&&&x\tabularnewline
~~&INDPRO&IP:Total index Industrial Production Index (Index 2012=100)&$5$&&x&x\tabularnewline
~~&IPFINAL&IP:Final products Industrial Production: Final Products (Market Group) (Index 2012=100)&$5$&&&x\tabularnewline
~~&IPCONGD&IP:Consumer goods Industrial Production: Consumer Goods (Index 2012=100)&$5$&&&x\tabularnewline
~~&IPMAT&Materials (Index 2012=100)&$5$&&&x\tabularnewline
~~&IPDMAT&Durable Materials (Index 2012=100)&$5$&&&x\tabularnewline
~~&IPNMAT&Nondurable Materials (Index 2012=100)&$5$&&&x\tabularnewline
~~&IPDCONGD&Durable Consumer Goods (Index 2012=100)&$5$&&&x\tabularnewline
~~&IPB51110SQ&Durable Goods:  Automotive products (Index 2012=100)&$5$&&&x\tabularnewline
~~&IPNCONGD&Nondurable Consumer Goods (Index 2012=100)&$5$&&&x\tabularnewline
~~&IPBUSEQ&Business Equipment (Index 2012=100)&$5$&&&x\tabularnewline
~~&IPB51220SQ&Consumer energy products (Index 2012=100)&$5$&&&x\tabularnewline
~~&CUMFNS&Capacity Utilization:  Manufacturing (SIC) (Percent of Capacity)&$1$&&&x\tabularnewline
~~&IPMANSICS&Industrial Production:  Manufacturing (SIC) (Index 2012=100)&$5$&&&x\tabularnewline
~~&IPB51222S&Industrial Production:  Residential Utilities (Index 2012=100)&$5$&&&x\tabularnewline
~~&IPFUELS&Industrial Production:  Fuels (Index 2012=100)&$5$&&&x\tabularnewline
~~&PAYEMS& Emp:Nonfarm All Employees: Total nonfarm (Thousands of Persons)&$5$&&&x\tabularnewline
~~&USPRIV& All Employees: Total Private Industries (Thousands of Persons)&$5$&&&x\tabularnewline
~~&MANEMP& All Employees: Manufacturing (Thousands of Persons)&$5$&&&x\tabularnewline
~~&SRVPRD&All Employees:  Service-Providing Industries (Thousands of Persons)&$5$&&&x\tabularnewline
~~&USGOOD&All Employees:  Goods-Producing Industries (Thousands of Persons)&$5$&&&x\tabularnewline
~~&DMANEMP&All Employees:  Durable goods (Thousands of Persons)&$5$&&&x\tabularnewline
~~&NDMANEMP&All Employees:  Nondurable goods (Thousands of Persons)&$5$&&&x\tabularnewline
~~&USCONS&All Employees:  Construction (Thousands of Persons)&$5$&&&x\tabularnewline
~~&USEHS&All Employees:  Education \& Health Services (Thousands of Persons)&$5$&&&x\tabularnewline
~~&USFIRE&All Employees:  Financial Activities (Thousands of Persons)&$5$&&&x\tabularnewline
~~&USINFO&All Employees:  Information Services (Thousands of Persons)&$5$&&&x\tabularnewline
~~&USPBS&All Employees:  Professional \& Business Services (Thousands of Persons)&$5$&&&x\tabularnewline
~~&USLAH&All Employees:  Leisure \& Hospitality (Thousands of Persons)&$5$&&&x\tabularnewline
~~&USSERV&All Employees:  Other Services (Thousands of Persons)&$5$&&&x\tabularnewline
~~&USMINE&All Employees:  Mining and logging (Thousands of Persons)&$5$&&&x\tabularnewline
~~&USTPU&All Employees:  Trade, Transportation \& Utilities (Thousands of Persons)&$5$&&&x\tabularnewline
~~&USGOVT&All Employees:  Government (Thousands of Persons)&$5$&&&x\tabularnewline
~~&USTRADE&All Employees:  Retail Trade (Thousands of Persons)&$5$&&&x\tabularnewline
~~&USWTRADE&All Employees:  Wholesale Trade (Thousands of Persons)&$5$&&&x\tabularnewline
~~&CES9091000001&All Employees:  Government:  Federal (Thousands of Persons)&$5$&&&x\tabularnewline
~~&CES9092000001&All Employees:  Government:  State Government (Thousands of Persons)&$5$&&&x\tabularnewline
~~&CES9093000001&All Employees:  Government:  Local Government (Thousands of Persons)&$5$&&&x\tabularnewline
~~&CE16OV&Civilian Employment (Thousands of Persons)&$5$&&x&x\tabularnewline
~~&CIVPART&Civilian Labor Force Participation Rate (Percent)&$2$&&&x\tabularnewline
~~&UNRATE&Civilian Unemployment Rate (Percent)&$2$&&x&x\tabularnewline
~~&UNRATESTx&Unemployment Rate less than 27 weeks (Percent)&$2$&&&x\tabularnewline
~~&UNRATELTx&Unemployment Rate for more than 27 weeks (Percent)&$2$&&&x\tabularnewline
~~&LNS14000012&Unemployment Rate - 16 to 19 years (Percent)&$2$&&&x\tabularnewline
~~&LNS14000025&Unemployment Rate - 20 years and over, Men (Percent)&$2$&&&x\tabularnewline
~~&LNS14000026&Unemployment Rate - 20 years and over, Women (Percent)&$2$&&&x\tabularnewline
~~&UEMPLT5&Number of Civilians Unemployed - Less Than 5 Weeks (Thousands of Persons)&$5$&&&x\tabularnewline
\bottomrule
\end{tabular}}
\caption{Data description\label{tab:data-descr1}}\end{center}}
\end{table}


==> data_desc2.tex <==
%latex.default(mc.cracken.2, file = "data_desc2.tex", title = "",     ctable = FALSE, rgroupTexCmd = "scshape", rgroup = rgroup,     n.rgroup = n.rgroup.1, caption = "Data description (cont.)",     label = "tab:data-descr1", size = "tiny", booktabs = TRUE,     numeric.dollar = TRUE, rowname = "", colnames = "", caption.loc = "bottom",     landscape = FALSE)%
\begin{table}[!tbp]
{\tiny
\begin{center}
\scalebox{0.8}{
\begin{tabular}{lllrlll}
\toprule
\multicolumn{1}{l}{\ }&\multicolumn{1}{c}{\ FRED.Mnemonic}&\multicolumn{1}{c}{\ Description}&\multicolumn{1}{c}{\ Trans I(0)}&\multicolumn{1}{c}{\ SMALL}&\multicolumn{1}{c}{\ MEDIUM}&\multicolumn{1}{c}{\ LARGE}\tabularnewline
\midrule
{\scshape Slow}&&&&&&\tabularnewline
~~&UEMP5TO14&Number of Civilians Unemployed for 5 to 14 Weeks (Thousands of Persons)&$5$&&&x\tabularnewline
~~&UEMP15T26&Number of Civilians Unemployed for 15 to 26 Weeks (Thousands of Persons)&$5$&&&x\tabularnewline
~~&UEMP27OV&Number of Civilians Unemployed for 27 Weeks and Over (Thousands of Persons)&$5$&&&x\tabularnewline
~~&AWHMAN&Average Weekly Hours of Production and Nonsupervisory Employees:  Manufacturing (Hours)&$1$&&&x\tabularnewline
~~&AWOTMAN&Average Weekly Overtime Hours of Production and Nonsupervisory Employees: Manufacturing (Hours)&$2$&&&x\tabularnewline
~~&HWIx&Help-Wanted Index&$1$&&&x\tabularnewline
~~&CES0600000007&Average Weekly Hours of Production and Nonsupervisory Employees:  Goods-Producing&$2$&&x&x\tabularnewline
~~&CLAIMSx&Initial Claims&$5$&&&x\tabularnewline
~~&HOUST&Housing Starts: Total: New Privately Owned Housing Units Started&$5$&&x&x\tabularnewline
~~&HOUST5F&Privately Owned Housing Starts: 5-Unit Structures or More&$5$&&&x\tabularnewline
~~&PERMIT&New Private Housing Units Authorized by Building Permits&$5$&&x&x\tabularnewline
~~&HOUSTMW&Housing Starts in Midwest Census Region (Thousands of Units)&$5$&&&x\tabularnewline
~~&HOUSTNE&Housing Starts in Northeast Census Region (Thousands of Units)&$5$&&&x\tabularnewline
~~&HOUSTS&Housing Starts in South Census Region (Thousands of Units)&$5$&&&x\tabularnewline
~~&HOUSTW&Housing Starts in West Census Region (Thousands of Units)&$5$&&&x\tabularnewline
~~&RSAFSx&Real Retail and Food Services Sales (Millions of Chained 2012 Dollars)&$5$&&&x\tabularnewline
~~&AMDMNOx&Real Manufacturers' New Orders:  Durable Goods (Millions of 2012 Dollars)&$5$&&&x\tabularnewline
~~&AMDMUOx&Real Value of Manufacturers' Unfilled Orders for Durable Goods Industries&$5$&&&x\tabularnewline
~~&BUSINVx&Total Business Inventories (Millions of Dollars)&$5$&&&x\tabularnewline
~~&ISRATIOx&Total Business:  Inventories to Sales Ratio&$2$&&&x\tabularnewline
~~&PCECTPI&Personal Consumption Expenditures: Chain-type Price Index &$6$&&x&x\tabularnewline
~~&PCEPILFE&Personal Consumption Expenditures Excluding Food and Energy&$6$&&&x\tabularnewline
~~&GDPCTPI&Gross Domestic Product: Chain-type Price Index&$5$&x&x&x\tabularnewline
~~&GPDICTPI&Gross Private Domestic Investment: Chain-type Price Index &$6$&&&x\tabularnewline
~~&IPDBS&Business Sector:  Implicit Price Deflator (Index 2012=100)&$6$&&&x\tabularnewline
~~&DGDSRG3Q086SBEA&Personal consumption expenditures:  Goods &$6$&&&x\tabularnewline
~~&DDURRG3Q086SBEA&Personal consumption expenditures:  Durable goods &$6$&&&x\tabularnewline
~~&DSERRG3Q086SBEA&Personal consumption expenditures:  Services &$6$&&&x\tabularnewline
~~&DNDGRG3Q086SBEA&Personal consumption expenditures:  Nondurable goods&$6$&&&x\tabularnewline
~~&DHCERG3Q086SBEA&Personal consumption expenditures:  Services:  Household consumption expenditures&$6$&&&x\tabularnewline
~~&DMOTRG3Q086SBEA&Personal consumption expenditures:  Durable goods:  Motor vehicles and parts&$6$&&&x\tabularnewline
~~&DFDHRG3Q086SBEA&Personal consumption expenditures:  Durable goods:  Furnishings and durable household equipment&$6$&&&x\tabularnewline
~~&DREQRG3Q086SBEA&Personal consumption expenditures:  Durable goods:  Recreational goods and vehicles&$6$&&&x\tabularnewline
~~&DODGRG3Q086SBEA&Personal consumption expenditures:  Durable goods:  Other durable goods&$6$&&&x\tabularnewline
~~&DFXARG3Q086SBEA&Personal consumption expenditures:  Nondurable goods:  Food and beverages purchased for off-premises consumption&$6$&&&x\tabularnewline
~~&DCLORG3Q086SBEA&Personal consumption expenditures:  Nondurable goods:  Clothing and footwear&$6$&&&x\tabularnewline
~~&DGOERG3Q086SBEA&Personal consumption expenditures:  Nondurable goods:  Gasoline and other energy goods&$6$&&&x\tabularnewline
~~&DONGRG3Q086SBEA&Personal consumption expenditures:  Nondurable goods:  Other nondurable goods&$6$&&&x\tabularnewline
~~&DHUTRG3Q086SBEA&Personal consumption expenditures:  Services:  Housing and utilities&$6$&&&x\tabularnewline
~~&DHLCRG3Q086SBEA&Personal consumption expenditures:  Services:  Health care&$6$&&&x\tabularnewline
~~&DTRSRG3Q086SBEA&Personal consumption expenditures:  Transportation services&$6$&&&x\tabularnewline
~~&DRCARG3Q086SBEA&Personal consumption expenditures: Recreation services&$6$&&&x\tabularnewline
~~&DFSARG3Q086SBEA&Personal consumption expenditures:  Services:  Food services and accomodations&$6$&&&x\tabularnewline
~~&DIFSRG3Q086SBEA&Personal consumption expenditures:  Financial services and insurance&$6$&&&x\tabularnewline
~~&DOTSRG3Q086SBEA&Personal consumption expenditures:  Other services &$6$&&&x\tabularnewline
~~&CPIAUCSL&Consumer Price Index for All Urban Consumers:  All Items&$6$&&x&x\tabularnewline
~~&CPILFESL&Consumer Price Index for All Urban Consumers:  All Items Less Food \& Energy&$6$&&&x\tabularnewline
~~&WPSFD49207&Producer Price Index by Commodity for Finished Goods &$6$&&&x\tabularnewline
~~&PPIACO&Producer Price Index for All Commodities &$6$&&&x\tabularnewline
~~&WPSFD49502&Producer Price Index by Commodity for Finished Consumer Goods &$6$&&&x\tabularnewline
~~&WPSFD4111&Producer Price Index by Commodity for Finished Consumer Foods&$6$&&&x\tabularnewline
~~&PPIIDC&Producer Price Index by Commodity Industrial Commodities &$6$&&&x\tabularnewline
~~&WPSID61&Producer Price Index by Commodity Intermediate Materials:  Supplies \& Components&$6$&&&x\tabularnewline
~~&WPU0561&Producer Price Index by Commodity for Fuels and Related Products and Power&$5$&&&x\tabularnewline
~~&OILPRICEx&Real Crude Oil Prices:  West Texas Intermediate (WTI) - Cushing, Oklahoma&$5$&&&x\tabularnewline
~~&WPSID62&Producer Price Index:  Crude Materials for Further Processing &$6$&&&x\tabularnewline
~~&PPICMM&Producer Price Index:  Commodities:  Metals and metal products:  Primary nonferrous metals&$6$&&&x\tabularnewline
~~&CPIAPPSL&Consumer Price Index for All Urban Consumers:  Apparel&$6$&&&x\tabularnewline
~~&CPITRNSL&Consumer Price Index for All Urban Consumers:  Transportation&$6$&&&x\tabularnewline
~~&CPIMEDSL&Consumer Price Index for All Urban Consumers:  Medical Care&$6$&&&x\tabularnewline
~~&CUSR0000SAC&Consumer Price Index for All Urban Consumers:  Commodities&$6$&&&x\tabularnewline
~~&CES2000000008x&Real Average Hourly Earnings of Production and Nonsupervisory Employees: Construction&$5$&&&x\tabularnewline
~~&CES3000000008x&Real Average Hourly Earnings of Production and Nonsupervisory Employees: Manufacturing&$5$&&&x\tabularnewline
~~&COMPRNFB&Nonfarm Business Sector:  Real Compensation Per Hour (Index 2012=100)&$5$&&&x\tabularnewline
~~&CES0600000008&Average Hourly Earnings of Production and Nonsupervisory Employees:&$6$&&x&x\tabularnewline
\bottomrule
\end{tabular}}
\caption{Data description (cont.)\label{tab:data-descr2}}\end{center}}
\end{table}


==> data_desc3.tex <==
%latex.default(mc.cracken.3, file = "data_desc3.tex", title = "",     ctable = FALSE, rgroupTexCmd = "scshape", rgroup = rgroup,     n.rgroup = n.rgroup.1, caption = "Data description (cont.)",     label = "tab:data-descr2", size = "tiny", booktabs = TRUE,     numeric.dollar = TRUE, rowname = "", colnames = "", caption.loc = "bottom",     landscape = FALSE)%
\begin{table}[!tbp]
{\tiny
\begin{center}
\scalebox{0.8}{
\begin{tabular}{lllrlll}
\toprule
\multicolumn{1}{l}{\ }&\multicolumn{1}{c}{\ FRED.Mnemonic}&\multicolumn{1}{c}{\ Description}&\multicolumn{1}{c}{\ Trans I(0)}&\multicolumn{1}{c}{\ SMALL}&\multicolumn{1}{c}{\ MEDIUM}&\multicolumn{1}{c}{\ LARGE}\tabularnewline
\midrule
{\scshape Policy rate}&&&&&&\tabularnewline
~~&FEDFUNDS&Effective Federal Funds Rate (Percent)&$2$&x&x&x\tabularnewline
\midrule
{\scshape Fast}&&&&&&\tabularnewline
~~&TB3MS&3-Month Treasury Bill: Secondary Market Rate (Percent)&$2$&&&x\tabularnewline
~~&TB6MS&6-Month Treasury Bill: Secondary Market Rate (Percent)&$2$&&&x\tabularnewline
~~&GS1&1-Year Treasury Constant Maturity Rate (Percent)&$2$&&x&x\tabularnewline
~~&GS10&10-Year Treasury Constant Maturity Rate (Percent)&$2$&&x&x\tabularnewline
~~&AAA&Moody's Seasoned Aaa Corporate Bond Yield (Percent)&$2$&&&x\tabularnewline
~~&BAA&Moody's Seasoned Baa Corporate Bond Yield (Percent)&$2$&&&x\tabularnewline
~~&BAA10YM&Moody's Seasoned Baa Corporate Bond Yield Relative to Yield on 10-Year Treasury&$1$&&&x\tabularnewline
~~&TB6M3Mx&6-Month Treasury Bill Minus 3-Month Treasury Bill, secondary market (Percent)&$1$&&&x\tabularnewline
~~&GS1TB3Mx&1-Year Treasury Constant Maturity Minus 3-Month Treasury Bill, secondary market&$1$&&&x\tabularnewline
~~&GS10TB3Mx&10-Year Treasury Constant Maturity Minus 3-Month Treasury Bill, secondary market&$1$&&&x\tabularnewline
~~&CPF3MTB3Mx&3-Month Commercial Paper Minus 3-Month Treasury Bill, secondary market&$1$&&&x\tabularnewline
~~&GS5&5-Year Treasury Constant Maturity Rate&$2$&&&x\tabularnewline
~~&TB3SMFFM&3-Month Treasury Constant Maturity Minus Federal Funds Rate&$1$&&&x\tabularnewline
~~&T5YFFM&5-Year Treasury Constant Maturity Minus Federal Funds Rate&$1$&&&x\tabularnewline
~~&AAAFFM&Moody's Seasoned Aaa Corporate Bond Minus Federal Funds Rate&$1$&&&x\tabularnewline
~~&BUSLOANSx&Real Commercial and Industrial Loans, All Commercial Banks&$5$&&&x\tabularnewline
~~&CONSUMERx&Real Consumer Loans at All Commercial Banks &$5$&&&x\tabularnewline
~~&NONREVSLx&Total Real Nonrevolving Credit Owned and Securitized, Outstanding&$5$&&&x\tabularnewline
~~&REALLNx&Real Real Estate Loans, All Commercial Banks&$5$&&&x\tabularnewline
~~&TOTALSLx&Total Consumer Credit Outstanding&$5$&&&x\tabularnewline
~~&TOTRESNS&Total Reserves of Depository Institutions &$6$&&x&x\tabularnewline
~~&NONBORRES&Reserves Of Depository Institutions, Nonborrowed&$7$&&x&x\tabularnewline
~~&DTCOLNVHFNM&Consumer Motor Vehicle Loans Outstanding Owned by Finance Companies&$6$&&&x\tabularnewline
~~&DTCTHFNM&Total Consumer Loans and Leases Outstanding Owned and Securitized by Finance Companies &$6$&&&x\tabularnewline
~~&INVEST&Securities in Bank Credit at All Commercial Banks &$6$&&&x\tabularnewline
~~&TABSHNOx&Real Total Assets of Households and Nonprofit Organizations&$5$&&&x\tabularnewline
~~&EXSZUSx&Switzerland / U.S. Foreign Exchange Rate&$5$&&&x\tabularnewline
~~&EXJPUSx&Japan / U.S. Foreign Exchange Rate&$5$&&&x\tabularnewline
~~&EXUSUKx&U.S. / U.K. Foreign Exchange Rate&$5$&&&x\tabularnewline
~~&EXCAUSx&Canada / U.S. Foreign Exchange Rate&$5$&&&x\tabularnewline
~~&S.P.500&S\&P's Common Stock Price Index:  Composite&$5$&&x&x\tabularnewline
~~&S.P..indust&S\& P's Common Stock Price Index:  Industrials&$5$&&&x\tabularnewline
~~&S.P.div.yield&S\& P's Composite Common Stock:  Dividend Yield&$2$&&&x\tabularnewline
\bottomrule
\end{tabular}}
\caption{Data description (cont.)\label{tab:data-descr3}}\end{center}}
\end{table}

